Performative Recommendation: Diversifying Content via Strategic Incentives

The primary goal in recommendation is to suggest relevant content to users, but optimizing for accuracy often results in recommendations that lack diversity. To remedy this, conventional approaches such as re-ranking improve diversity by presenting more diverse items. Here we argue that to promote inherent and prolonged diversity, the system must encourage its creation. Towards this, we harness the performative nature of recommendation, and show how learning can incentivize strategic content creators to create diverse content. Our approach relies on a novel form of regularization that anticipates strategic changes to content, and penalizes for content homogeneity. We provide analytic and empirical results that demonstrate when and how diversity can be incentivized, and experimentally demonstrate the utility of our approach on synthetic and semi-synthetic data.

==> synthetic_exp_plots/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Through the lens of performativity,
our paper studies how a learning system can incentivize content creators to collectively form a more diverse inventory of items for recommendation.
In this, we challenge the conventional view that diversity is merely a matter of which items to present (and which not),
and argue that to fundamentally rectify the predisposition of modern recommendation systems to homogenize content,
learning must (i) recognize that content \emph{changes} over time,
in part due to the strategic behavior of content creators, and
(ii) capitalize on its power shape incentives and steer towards diversity.
Our work joins others in taking a step towards studying recommendation systems as complex ecosystems in which users, creators, and the system itself act and react to promote their own goals and aspirations.
From a learning perspective, this requires us to rethink the role that predictions play in the recommendation process,
and consider its implications on user welfare.

\todo{limitations; future work}

% This paper examines how the content creator's strategic response can impact the diversity of recommendation lists. We identified factors that affect diversity and analyzed how they might affect it. According to our findings, strategic responses to RS might increase diversity, but might damage it as well. 
% % A key property that affects diversity is the willingness of the item creator to be relevant to multiple users (who may have varying preferences). By using this property we propose framework that exploit the strategic changes that made on items to increase diversity.
% We propose a framework that exploit the strategic changes that made on items to increase diversity.
% We tested our framework on Yelp dataset and found that our method might improve significantly the diversity. \red{A future work might use the difference in user preference} to improve other important aspects of recommendation system such as novelty \red{add more..}   


==> synthetic_exp_plots/abstract.tex <==
The primary goal in recommendation is to suggest relevant content to users,
but optimizing for accuracy often results in recommendations that lack diversity.
To remedy this, conventional approaches
such as re-ranking improve diversity
by \emph{presenting} more diverse items.
Here we argue that to promote inherent and prolonged diversity, the system must encourage its \emph{creation}.
Towards this, we harness the performative nature of recommendation,
and show how learning can incentivize
strategic content creators to create diverse content.
Our approach relies on a novel form of regularization that anticipates strategic changes to content, and penalizes for content homogeneity.
We provide analytic and empirical results that demonstrate when and how diversity can be incentivized,
and experimentally demonstrate the utility of our approach on synthetic and semi-synthetic data.


% Recommendation systems are designed to provide users with a list of relevant items. Several studies have indicated, however, that relevance alone is not sufficient for recommendation systems to satisfy users. A recommendation list should have diversity as one of its most important properties. While previous works have attempted to increase the diversity of the recommendation list, it neglected the actions that strategic content creators might take to achieve a higher score. This study examines how content creators' strategic behavior affects the diversity of recommendation lists and proposes a framework that employs look-ahead regularization to encourage content creators to engage in more diverse product development.

==> synthetic_exp_plots/analysis.tex <==
% \begin{figure}[ht]
%   \includegraphics[width=\linewidth]{Diversification analysis using user vectors.pdf}
%   \caption{The right side shows that it doesn't matter how we choose the two embedding vectors that aren't shared between the two items. Both best responses are very close to each other, which leads to a small diversity. On the other hand, we can see in the left side that when the system chooses the user embedding smartly, the summation of the shared vectors can be zero and thus only the two non-shared vectors influence which can lead to maximization of diversity.}
%   \label{control_embd}
% \end{figure}
% \label{sec:analysis}


\section{Diversity via Strategic Incentives}
% - system can incentivize 
% - controls u
% - Q: when can it be used to generate diversity?
% - to answer, simplify and consider minimal setting
% - [details]
% - short answer: need diversity to create diversity
% - role of stage 1

\label{sec:diversity_strategic_incentives}
The reliance of the utility of content creators on the learned $f$
provides the system with potential power for shaping incentives,
and here we study when this potential can materialize.
% The system's control is expressed in its ability to determine user embeddings $u_i$, and we will be interested in how this control can translate to diversification incentives.
To addresses this question, we begin by considering a simplified setting 
% aimed at preserving the minimal structure necessary .
that focuses exclusively on maximizing diversity,
for a single time step with no cost restrictions (i.e., set $\alpha=0$).
This removes any potential constraints on $u_i$ that may arise from accuracy considerations,
and serves as a convenient substitute for lengthy strategic dynamics. %\looseness=-1

\extended{In Appendix \ref{apx:empirical_generalization_full_overlapping} we empirically show that this is indeed representative of $\alpha>0$ over time (absent retraining).}

Our main object of interest in the analysis is the recommendation graph $G$,
viewed as input to the learning algorithm.\footnote{Put differently, we study how
our focal task of $2^{\text{nd}}$-stage recommendation
is effected by the outputs of $1^{\text{st}}$-stage algorithms.}
As we show, whether diversification through incentivization is possible (or not)
depends on properties of the graph.
We first consider the graph of a single item list $X$ and all related users (i.e., users $u_i$ for which some $x_j \in X_i$ is also in $X$),
and then proceed to general graphs over multiple lists.

We begin with a negative result for single lists. %, and shows when diversity in unattainable.
\begin{proposition}
\label{prop:Full_users_overlap}
Let $X=\{x_1,x_2\}$.
% $x_1$ and $x_2$ be two items with
If both items have
fully overlapping users
(i.e., $U_1 = U_2$), then for any $f$, %$\diversity(x_1,x_2)=0$.
% $\Delta_f(x_1) = \Delta_f(x_2)$,
$\diversity(X^f,\r^f)=0$.
Hence, diversity cannot be incentivized.
% which implies that
% (i.e.,  diversity between $\Delta_f(x_1)$ and $\Delta_f(x_2)$ is zero).
\end{proposition}
% \red{
% prop 1 and prop2 consider $div(X)$ for single list $X$.
% we think of $x_1,x_2$ as items in a list $X=\{x_1,x_2\}$, and consider all users who have them in their lists. we say "div between", but actually mean in the list (prop3 will be about multiple lists)}
Proof in Appendix \ref{apx:proof_full_users_overlap}.
% \todo{add to appendix empirical experiments that consider $\alpha>0$ and multiple time-steps. mention and reference here.}
Essentially, Prop. \ref{prop:Full_users_overlap} states that since user representations drive content creator interests,
similar users lead to similar incentives.
This results in identical modified items,
$\Delta_f(x_1) = \Delta_f(x_2)$,
and hence zero diversity.
% \todo{operational conclusion}
Extending the result to larger item sets and multiple users is straightforward, and implies the following:
if the same list of potentially-relevant items is associated
exclusively with the same group of users, 
then strategic behavior is bound to nullify diversity entirely---regardless of any system efforts.
% if a group of users shares the same exclusive list of potentially-relevant items,
% then recommendation cannot be used to improve diversity.
% diversity is destined to dissipate, regardless of system efforts.

Conversely, Prop. \ref{prop:Full_users_overlap} hints that to diversify items,
it is necessary to start out with some initial variation in the assignment of users to items. But how much user variation is needed?
Our next result shows that for a single item list, when no other considerations are present,
minimal differentiation in users is sufficient for obtaining maximal item diversity.
\begin{proposition}
\label{prop:diff_users_max_div}
Let $X=\{x_1,x_2\}$.
% Let $x_1$ and $x_2$ be two items whose
If $U_1,U_2$ differ only in a single user,
i.e., if $U_1 = U\cup\{u_1\}$ and $U_2 = U\cup\{u_2\}$ for some $U,u_1,u_2$,
% i.e., $U_1 = U \cup \{u_1\}$ and $U_2 = U \cup \{u_2\}$ for some $U$ and $u_1,u_2$.
then there exists an $f$
which obtains maximal diversity;
and if $|U|>1$, then 
$\diversity(X^f,\r^f)=1$.
%, then $\diversity(X^f,\r^f)=1$.
% diversity between $\Delta_f(x_1)$ and $\Delta_f(x_2)$ \blue{is one, i.e.,} is maximal.
\end{proposition}  
% \todo{make it clear that each set has a distinct item. consider stating that if $|U_1 \cap U_2|\ge2$ then div=1, otherwise max possible div is less than one (but still attainable)}
The proof is constructive, and appears in Appendix \ref{apx:proof_diff_users_max_div}.
Prop. \ref{prop:diff_users_max_div} shows that,
under lenient conditions,
incentivization can drive diversity to its greatest possible extend.
Generally, and under more realistic considerations (e.g., accuracy and cost constraints),
we expect that greater differentiation is likely necessary,
even for lower gains in diversity.

We now  move to considering graphs for %a full graph $G$ consisting of 
multiple item lists.
This introduces dependencies:
if some item $x_j$ appears in two distinct but partially-overlapping user lists $X_i,X_{i'}$,
then this restricts the possible values that the embeddings $u_i,u_{i'}$ can take.
As such, Prop. \ref{prop:diff_users_max_div} cannot simply be applied
to each list in $G$ independently, since $f$ cannot be tailored to maximize diversity for $X_i$ without affecting $X_{i'}$, for which $f$ may not be optimal.
% \todo{show this!}
Our final result shows that, despite such dependencies,
significant diversity is still attainable.

% \todo{prop 3 needs to talk about non-overlapping lists - otherwise prop2 applies}

\green{
% prop 3
% - prop2 considers a single (arbitrary) item list $X=\{x_1,x_2\}$ (this is what we measure div on) and its associated users
% - move to focus on (i) entire graph, and (i) average over users
% - this introduces dependencies: system can't now set $u_i$ to promote div of a target list (as before), since now this can affect multiple lists.
% % - (prop2 it was an arbitrary item listl now it has to be user's lists, and for all users)
% - hence, can't just `apply' prop 2
}
\begin{proposition}
\label{prop:div_multi_list}
Let $K=2$, then 
for any $\epsilon>0$ and any $N$,
there exists a graph $G$ over $N$ distinct lists
and a corresponding $f$ s.t. the average diversity is at least
$(1-\epsilon)(1-3/N)$.
% \begin{equation}
% \label{eq:div_multi_list}
% \diversity>(1-\epsilon)(1-3/m)
% \end{equation}
\end{proposition}
Proof in Appendix \ref{apx:proof_div_multi_list}, and relies on a construction that
simultaneously (i) decouples users across lists, and
(ii) permits maximal diversity within lists.
Prop. \ref{prop:div_multi_list} shows that
the potential for incentivizing for diversity grows towards the near-optimal value of $1-\epsilon$ quickly,
in term of the number of lists $N$---and to the degree that the graph permits.

% \red{
% - elaborate on why this is not trivial
%   - for example, chain bip graph gives max div apx 90 degrees (and not 180)
% % - proof: clever decoupling of users
% }

% \blue{here we showed that it is theoretically possible to create high diversity through incentivization. next we show empirically that it is also possible in practice---and our learning approach achieves this---in increasingly realistic scenarios (=no direct control of $G$, non-zero costs, etc).}

% \green{\rule{\columnwidth}{3pt}}
%==============================================================================

% The strategic modifications that made by items creator might affect the diversity. As we show next those changes can both harm and benefit the diversity. In this section we theoretically analyze which factors might affect the diversity. To examine the effect on diversity, we simplify the setup and look for RS that care only about diversity (or use an extremely large $\lambda$).
% \nir{need to say here that you will be looking at a simplified setup where you don't care about ndcg, only diversity - and justify why this is ok to do. say that this gives the system complete flexibility in choosing embeddings $u$; and that when you do add ndcg to the objective, then this `constrains' embeddings to provide good ndcg}

% \nir{also say why looking at $\alpha=0$ is interesting, and that its a simplification of the dynamic process (?) that reduces it to a single step.} \itay{That not very accurate. As I show in the synthetic exp, when $\alpha$ is high it might help the RS to create diversity but it might take time. It is simplify only if the model doesn't train again during the different period. }

% \subsection{Overlapping potential users between different items}

% \nir{is the goal of this section to give insight as to the role of the bipartite graph in enabling the creation of diversity? or something more general? or something else completely...?}

% \begin{proposition}
% \label{prop:Full_users_overlap}
% Let $x_1$ and $x_2$ be two items with exactly the same set of users i.e $U_{x_1} = U_{x_2}$. If there is no limitation on feature changing ($\alpha=0$) the diversity between two items is 0. 
% \end{proposition}
% \nir{is this also what will happen if $\alpha>0$ but you allow multiple time steps? will it approach div=0 in the limit (of time)?} \itay{Yes. I tested it empirically but I don't have mathematical proof.}
% \todo{push proof to appendix}
% \begin{proof}
% As both items have the same set of users, the normalized average of users embedded (i.e equation \eqref{avg_u}) is the same for both items. We denote normalized average of users embedded by $v$. Since there is no limitation for the modification $\alpha=0$ the best response (according to equation \eqref{eq:best_response_close}) is to change the item vector feature to $v$. 
% As a result both item will be changed to the same point which means dissimilarity of 0 between them.
% \end{proof}
% As proposition 1 shows, there is minimize diversity if two items appeal to the same users and there is no limitation to the cost. When $\alpha$ is not 0, it may take time for items to reach 0 diversity, since their ability to change is restricted. If the RS is fixed (trains only once), users embedding do not change and over time small diversification is caused by repeated strategic changes.  
% The next question is what is minimum number of non-shared users to allow for maximum diversity. Consider two items $x_1$ and $x_2$ with shared users group $U$ and two users A and B which user A contains $x_1$ in his recommendation list but not $x_2$ and users B contains $x_2$ but not $x_1$. If the embedding of the users in $U$ has small diversity and $U$ is very large group, the average of the users in $U_{x_1}$ and the average of users in $U_{x_2}$ will be close to the average of $U$. Therefore we can expect the items best response to be close to each other as figure \ref{control_embd} right shows. we note that it doesn't matter what is the embedding of users A and user B since $U$ is very large group. However, since the RS has the ability to choose the user embedding, it might choose the embedding of the users in $U$ in a manner that their sum will be close to $0$, the best response of each item is determine only by the not common user. Consequently, if $\sum_{u \in U}u = 0$ and $u_A = -u_B$ we get maximize diversity (figure \ref{control_embd}). In this example we demonstrated how the RS can control users embedding in order to create diversity. But we might get poor \NDCG since we ignore the true preference of the users.
% \begin{proposition}
% \label{prop:rec_list_len2}
% In RS with $m$ users and $m$ items we define the recommendation list for all user to be: user $i$ where $1\le i < m$ the items $x_i, x_{i+1}$ and for the $m$'th user $x_m, x_1$. For every $\epsilon \in (0, 1)$ exist $m$ that satisfy $\DIV(\Delta(X), U)>\epsilon$.  
% \end{proposition}

% % \begin{proposition}
% % \label{prop:rec_list_len2}
% % We denote in $2\le m$ the number of users and the number of items in the system. The recommendation list for all user $1\le i < m$ is the items $x_i, x_{i+1}$ and for the $m$'th user $x_m, x_1$. For every $\epsilon \in (0, 1)$ exist $m$ that satisfy $\DIV(\Delta(X), U)>\epsilon$.  
% % \end{proposition}
% \nir{you can't start with `let $m$', and end with `then exists $m$' (because you've fixed $m$ initially). what do you want to fix, and what do you want to vary?}\itay{I want to vary $m$ but first I want to define it. Is it better now?}
% \begin{proposition}
% \label{prop:clic size}
% % Given two groups of users in size $m$ $U_1 = {u_i}_{i=1}^m$ and $U_2 = {u_i}_{i={m+1}}^{2m}$. All the users in $U_1$ have the same items in the recommendation list and all the users in $U_2$ has the same items in their recommendation list. There is no item that shared between users from different groups. By choosing two users from different group and switch items  
% \red{Let $2 \le m$ be the number of users and $l$ the number of items in the recommendation list. The recommendation list of user $i < \frac{m}{2}$ is $\{x_j\}_{j=1}^l$ and the recommendation list for user $i \ge \frac{m}{2}$ is $\{x_j\}_{j=l+1}^{2l}$.For every $\epsilon \in (0, 1)$ exist $m$ that given item replacement (i.e switching between two users different items) the system is able to get $\DIV(\Delta(X), U)>\epsilon$.} 
% \end{proposition}

% Note that the above analyse assumes not cost limitation on the movement. If there is limitation Our strategic model might use it in order to create diversity (see section 5).

% % \begin{proposition}
% % \label{prop:rec_list_len_l}
% % Let $2 \le m$ be the number of users in the system and $l$ then number of items in the recommendation list. the recommendation list for all user $1\le i < m$ is the items $x_i, x_{i+1}$ and for the $m$'th user $x_m, x_1$. For every $\epsilon \in (0, 1)$ exist $m$ that satisfy $\ILD(X, U)>\epsilon$.  
% % \end{proposition}

% * The importance of the 'Bilateral graph'. How click might prevent diversity.. (proposition 1)\\
% * One change in two click might create great difference if RS think strategically. two option too look at it: 1. arrows are in the same direction (pretty much) and low diversity (might get very high ndcg). 2. arrows cancel each other diversity get higher (ndcg suffers). proposition 2 and maybe 3\\

% * more changes higher diversity proposition 3 (or 4 depends how we counts).\\
% * Option: analyse some expression of diversity\\
% * If we had cost would it matter? why small budget (high cost factor or high $\alpha$) might be better for diversity (Long term planning). does ndcg suffer? when? (not always suffer..)  

==> synthetic_exp_plots/intro.tex <==
\section{Introduction}
\label{sec:intro}

% \red{
% papers to cite in intro:
% - Artificial intelligence, music recommendation, and the curation of culture: A white paper \\
% - Building Human Values into Recommender Systems: An Interdisciplinary Synthesis
% }

Recommendation has become a key driving force in determining what content we are exposed to,
and ultimately, which we consume \citep{mackenzie2013retailers,ursu2018power}.
But despite their commercial success,
a well-known shortcoming of modern systems is that recommendations tend to be insufficiently diverse,
with homogeneity of content becoming more pronounced over time;
this has been a longstanding issue in the field for over two decades \citep{carbonell1998use,bradley2001improving}.
Diversity is important in recommendation not only for improving recommendation quality \citep{vargas2014improving,kaminskas2016diversity}
and user satisfaction \citep{herlocker2004evaluating,ziegler2005improving,mcnee2006being,hu2011helping,wu2018personalizing,dean2020recommendations},
but also because a lack of diversity can lead to inequity across content creators,
which often hurts the `long-tail' of non-mainstream suppliers
\citep{yin2012challenging,burke2017multisided,singh2018fairness,abdollahpouri2019unfairness,mladenov2020optimizing,wang2021user}.
% thus reducing overall efficiency.
From the perspective of the recommendation platform,
an inability to diversify content translates into an inability
to utilize the full potential that lies in
the natural variation of user preferences
for promoting system goals
\citep{anderson2006long,yin2012challenging}.
This has lead to widespread interest in developing methods for  making recommendations more diverse \citep{kunaver2017diversity}. %;
% see \citet{kunaver2017diversity} for an extensive survey.

The common approach for diversifying recommendations
% are base on a post-processing procedure that reranks 
is to apply some post-processing procedure 
that re-ranks the output of a conventionally-trained ranking model---which is optimized for predicting user-item relevance---to be more diverse,
for example by traversing the ranked list and removing items which are similar to higher-ranked items
\citep{carbonell1998use,ziegler2005improving,sha2016framework}.
This simple heuristic approach has been shown to be quite effective---at least when considering a \emph{given} ranked list, and at one point in time.
But recommendation is inherently a dynamic process:
here we argue that post-hoc methods may not suffice for promoting diversity in the long run.\looseness=-1
% % dynamic nature of recommendation environments,
% here we argue that re-ranking (and similar approaches)
% may be insufficient for promoting diversity
% in the long run.
% % that is prolonged and sustained.

To see why, 
consider that re-ranking (and similar approaches)
are designed to diversify the \emph{presentation} of content---not content itself.
Presenting diverse content may help in the specific instance it targets,
but does not change the pool of available items,
nor does it account for the downstream affects of recommendation.
% It is unclear, however, whether this approach permits sustained diversity;
% the fact that (non)diversity still remains to be a major issue in recommendation
% likely suggests otherwise.
Recent work has shown that optimizing recommenders to \emph{predict} well can lead to undesired outcomes, including content homogenization \citep{chaney2018algorithmic}\todo{add more};
here we argue that rearranging items to create the appearance of diversity does not remedy this.

As an alternative, we propose to encourage the \emph{creation} of diverse content, so that 
the set of available items becomes inherently more diverse.
In this way, we aim to target the cause---rather than the symptom.
Our main observation is that content is shaped by \emph{content creators}, who seek to maximize exposure to their items \citep{ben2020content,hron2022modeling},
and hence likely to modify content in ways which promote their item's predicted relevance (or `score').
Since the goal of learning is to infer such scores,
this gives the learning system leverage in shaping the 
incentives of content creators.
Here we propose to utilize this power to incentivize
for the creation of more diverse content.
% In this way, rather than targeting the symptom,
% our work aims directly for the cause.

Towards this, 
we draw connections to the related literature on strategic 
% \blue{classification/regression/learning} \tocite,
learning 
\citep{bruckner2012static,hardt2016strategic},
and model content creators as gaining utility from the score given to their items by the learned predictive model.
Content creators can then improve their utility
by strategically modifying their items to obtain a higher score. %\footnote{\blue{This is similar in spirit to search engine optimization (SEO).}}
Thus, a learned predictive model determines not only what items are recommended to which users---but also creates incentives for content creators,
which can promote change
\citep{ben2018game,jagadeesan2022supply}.
This provides the system with the potential power to steer
the collection of renewing items---over time, 
and with proper incentivization---towards diversity \citep{hardt2022performative}.

% In this work, we study the question of when and how the system can utilize its power to incentivize?

% When can the system effectively exercise its power to incentivize, and how?
To study when and how the system can effectively exercise its power,
%  to incentivize the formation of long-term diversity,
we cast recommendation as an instance of
\emph{performative prediction} \citep{perdomo2020performative},
which subsumes and extends strategic learning to a temporal setting where
repeated learning causes the underlying data to shift over time.
% a recently proposed framework for modeling how 
% the repeated deployment of a learned predictive rule can cause the underlying data to shift in response to predictions and over time.
Focusing on retraining dynamics
\tocitec{PP papers with retraining},
we study when and how learning
can be used to incentivize the creation and preservation of diversity.
In retraining, our only means for driving incentivizes derives from 
\emph{how} we retrain, i.e., from our criterion for choosing the predictive model at each time step.
Since retraining aims for models that are predictively accurate,
our goal will be to provide recommendation that are accurate \emph{and} diverse.
But diversity and accuracy can be at odds;
hence, we seek to understand how they relate, % between accuracy and diversity,
and to propose ways in which their tradeoff can be optimally exploited.

% if we seek to maintain a certain level of accuracy---how much flexibility
% do we have for encouraging diversity?


% From an algorithmic perspective,
% the literature on performative prediction focuses primarily on dynamics
% that result from applying \emph{repeated risk minimization} (RRM),
% also known simply as `retraining'.
% Periodic retraining is a common approach for learning in the presence of temporally varying data which ensures that, to some degree, accuracy is maintained throughout.
% Although more elaborate approaches for dynamic recommendation exist,
% the benefit of RRM is that it provides a simple means to constrain the system
% to predict well at each time point,
% and in this way avoid arbitrary exploration---which can be undesired, unethical, or even illegal in human-facing systems \citep{milano2020recommender,flick2016informed}.
% In light of this, here we follow suit,
% and intentionally remain within the supervised learning paradigm.
% From a strategic modeling perspective,
% this implies that our only means for driving incentivizes
% derives from the our choice of \emph{how} to retrain.

% This leads us to ask:
% when can retraining incentivize the creation and preservation of diversity, and how?
% To study this question,
% To answer this,
We begin with a basic analysis demonstrating the mechanisms through which incentives and diversity relate within our setup.
We then propose a learning objective that allows to balance ranking accuracy
(and in particular NDCG) with diversity through a novel form of regularization,
which we use to maximize diversity under accuracy constraints.
% (in a similar spirit to \citet{angelopoulos2022recommendation}).
Our proposed diversity regularizer has two main benefits.
First, it is differentiable,
and hence can be optimized using gradient methods.
Second, it can be applied to \emph{strategically-modified inputs};
this equips our objective with the ability to anticipate the
strategic responses of content creators,
and hence, to encourage predictive rules that incentivize diversity.
Our proposed strategic response operator is also differentiable;
thus, and using recent advances in differentiable learning-to-rank,
our entire strategic learning objective becomes differentiable,
and can be efficiently optimized end-to-end.

Using our proposed learning framework, we empirically demonstrate
how properly accounting for strategic incentives can improve diversity---and how neglecting to do so can lead to homogenization.
We begin with a series of synthetic experiments, each designed to study a different aspect of our setup, such as the role of time,
the natural variation in user preferences,
and the cost of applying strategic updates.
We then evaluate our approach in a semi-synthetic environment 
using real data (Yelp restaurants) and simulated responses.
Our results demonstrate the ability of strategically-aware retraining to bolster diversity,
and illustrate the importance of incentivizing the creation of diversity.

\todo{add illustration of dynamics (=updates+retraining) for myopic vs. strategic}

\extended{
\paragraph{Contributions.}
Our work makes the following contributions:
\begin{itemize}
\item ...
\end{itemize}
}


%=============================================================================
%=============================================================================


==> synthetic_exp_plots/learning_setup.tex <==
\section{Problem Setup}
\label{sec:Setup}
% \subsection{RS main goal recommend relevant items}

Our setup considers a recommendation platform consisting of $m$ users and $n$ items.
Items are described by feature vectors $x_j \in \R^d$, $j \in [n]$,
and each item $x_j$ is owned by a (strategic) content creator $j$.
The goal of the system is to learn latent vector representations $u_i \in \R^d$
for each user $i \in [m]$ that are useful for recommending relevant items.
As in \citet{hron2022modeling}, we assume all features
are constrained to have unit $\ell_2$ norm, $\|u\| = \|x\| = 1$
(i.e., lie on the unit sphere).
% i.e., lie on the $\ell_2$ unit ball $B_2$,
This ensures equal treatment across items (by the system)
and users (by content creators),
and prevents features from growing indefinitely due to strategic updates.


The system makes recommendations by ranking items for each user $i$ using a personalized score function $f_i(x)$ as:
\begin{equation}
\r_i = \rank(f_i(x_1),\dots,f_i(x_n))
\,\,\quad \forall i \in [m]
\end{equation}
where $f_i(x) = f(x;u_i)$ rely on learned user representation vectors $u_i$.
For a list of items $X$ we denote in shorthand $\r_i=\rank(f(X;u_i))$.
As in most works on strategic learning
\citep[e.g.,][]{hron2022modeling, jagadeesan2022supply, carroll2022estimating},
we consider linear score functions $f(x;u_i) = u_i^\top x$.
Overall, the goal of the system is to learn good $f_1,\dots,f_n$ from data,
where $u_1,\dots,u_n$ are the learned parameters.

\extended{Linear scores are used extensively in the strategic learning literature
since the learned $u$ can be interpreted as estimated user preferences
(in line with expected utility theory \citep{mas1995microeconomic}),
and since they permit tractable strategic responses. %\footnote{Despite using linear scores,  responses in our setting are \emph{not} linear due to graph dependencies and normalizing constraints.}
In recommendation, linear models have been shown to be sufficiently expressive in multiple settings \citep{ferrari2019we}.
Despite the linearity of $f$,
our learning problem is highly non-linear 
due to norm constraints, strategic responses,
and the ranking objective.}


\paragraph{Learning objective.}
% The primary goal of the system is to recommend relevant items.
We measure ranking quality using the standard measure of NDCG evaluated on the top $k$ items,
defined as follows.
Consider a list of items with relevance scores $\y=(y_1,\dots, y_n)$.
Let $\r=(r_1,\dots,r_n)$ be a ranking,
and denote by $\r(\ell)$ the index of the $\ell^{\text{th}}$-ranked item in $\r$.
Then the top-$k$ discounted cumulative gain (DCG) is: %\looseness=-1
\begin{equation}
\label{eq:DCG@k}
\DCGk(\y, \r) = \sum_{\ell=1}^k\frac{2^{y_{\r(\ell)}}-1}{\log(1+\ell)}
% \DCGk(\y, \r) = \sum_{\ell=1}^K \1{r_\ell \le k} \frac{2^{y_\ell}-1}{\log(1+r_\ell)} 
\end{equation}
where $2^{y_j}-1$ measures the `gain' in relevance from having item $j=r(\ell)$ in the top $k$, and $\log(1+\ell)$ `discounts' its rank.
NDCG is then obtained by normalizing relative to the optimal ranking
$\r^* = \argmax_{\r} \DCGk(\y,\r)$.
The primary goal of the system is therefore to learn
%score functions $f_{u_i}$, parameterize by
user representations $\{u_i\}_{i=1}^n$
that optimize average top-$k$ NDCG:
\begin{equation}
\max_{u_1,\dots,u_m} \frac{1}{m} \sum_{i=1}^m
\NDCGk(\y_i,\r_i)
\end{equation}
where $\r_i$ is the ranking of items for user $i$ according to $f(x;u_i)$.
% $\r_i = \rank(f(X_i;u_i))$ is the ranking of items in $X_i$ for user $i$.
% and for a list of items $X=\{x_1,\dots,x_K\}$ we denote in shorthand $\r_i=\rank(f(X;u_i))$.
For learning, we will assume that the system has access to relevance labels
$y_{ij}$ for some user-item pairs $(i,j)$,
and the goal is to generalize well to other pairs.

\paragraph{Item diversity.}
In addition to ranking accuracy,
we will also be interested in measuring and promoting diversity across recommended items. Here we focus on intra-list diversity
\citep{ziegler2005improving,vargas2011rank,antikacioglu2019new}
and use cosine similarity as a metric,
% $\cos(x,x') = x^\top x' / \|x\|\|x'\|$
$\cos(x,x') = \frac{x^\top x'}{\|x\|\|x'\|}$
which is appropriate for comparing unit-norm features
\citep{ekstrand2014user, hron2022modeling}.\footnote{Since features are normalized, we have $\cos(x,x') = x^\top x'$.}
For a list of items $X=(x_1,\dots,x_K)$ and corresponding ranking $\r$,
diversity for the top-$k$ items is defined as:
\begin{equation}
\label{eq:divk}
\divk(X,\r) = 
% \diversity(X,\r) = 
\frac{1}{k(k-1)}
\sum_{j,\ell=1}^k 1-\cos(x_{\r(j)},x_{\r(\ell)})
\end{equation}
% We will use Eq. \eqref{eq:diversity} to meausre diversity, and explictly optimize it.
which takes values in $[0,1]$ \citep{smyth2001similarity}.



\paragraph{Recommendation graph.}
In our setting, each user $i$ is associated with a list of $K_i$ potentially-relevant items, 
denoted $X_i \subseteq [n]$, 
and the system's goal is to choose a subset of $k\le K_i$ items to recommend as a ranked list.\extended{\footnote{This is also known as 
second-stage recommendation; see e.g. \citet{wang2022fairness}. \todo{refs within}}}
% We will write
% %hence use $f(X_i;u_i) = (f(x_1;u_i),\dots,f(x_{K_i};u_i))$
% $\r_i=\rank(f(X_i;u_i))$ as the ranking of $X_i$ for user $i$.
Since the same items can appear in multiple lists,
it will be useful to consider users and items through a bipartite graph $G=(U,X,E)$, where $(i,j) \in E$ if item $j$ is in user $i$'s list of candidate items.\footnote{For simplicity we assume $G$ is fixed, but note our framework also supports time-varying graphs.}
We will also denote $U_j = \{ i \in [m] \mid (i,j) \in E \}$
and $m_j = |U_j|$.
% Under this formulation, recommendation can be cast as finding a relevant subgraph $G_{\text{rec}} \subset G$ with $\deg(i)=k$ for all $i \in [m]$.
As we will see, the graph plays a key role in determining the system's potential for encouraging diversity.


% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=0.3\textwidth]{non_strategic_vis.png} \quad
% 	\includegraphics[width=0.3\textwidth]{strategic_response.pdf} \quad
% 	\includegraphics[width=0.3\textwidth]{strategic_incentive.pdf}
% 	\caption{\textbf{(Left)}
% 	Top 2 example of how model changes user features projection according to lambda. In red user preference maximize ndcg $u = 2x_2 + x_1$ and the rank order is 2, 3, 1 (2 is in the top of the list) and in blue maximize the diversity according cosine similarity $u=-x_1 - \frac{x_2}{2}$ and the order is 3, 1, 2. We can see that the angles between point 3 and point 1 is the maximize angle in the plot and thus maximize the diversity. Each dotted line shows the projection of point on $u$ vector.
% 	\textbf{(center)} Item creator's best response. The original item features are marked as x. The ideal vector for changing an item to is v. However, best response depends on \red{cost factor} $\alpha$. By lowering $\alpha$, we see that the item's best response becomes closer to v. \textbf{(right)} The true vector preference of user is $u$. The RS find vector $\hat{u}$ as the user embedding that maximize NDCG. Since item $x_1$ also in the recommendation list of user 1 and item $x_2$ is in the recommendation list of user 2, the RS can change the vector embedding of those two user and increase dissimilarity of $x_1$ and $x_2$.      
% 	}
% 	\label{fig:user_embd}
% \end{figure*}

\begin{figure*}[t]
	\centering{
	\includegraphics[width=0.85\textwidth]{illust-crop.pdf}
	}
	\caption{
	\textbf{(A)} \textbf{Tradeoff between accuracy and diversity:} Consider three items with high ({\color[RGB]{84,130,53}$\huge{\bullet}$}),  
	medium ({\color[RGB]{255,192,0}$\huge{\bullet}$}), and low
	({\color[RGB]{192,0,0}$\huge{\bullet}$}) ratings,
	and set $k=2$.
	\textbf{(A1)} For a learned user embedding $u_i$,
	projected item scores (empty circles) are ordered correctly (so $\NDCGk$ is high), but the resulting diversity is low (blue circular sector).
	\textbf{(A2)} Learning a different $u'_i$ (note the flipped orientation) results in lower NDCG,
	but diversity is now maximal.
	\textbf{(B)} \textbf{Creating diversity with strategic incentives:}
	Consider two items %$x_1,x_2$
	and three users %$x_0,x_1,x_2$
	connected by the graph $G$.
	Initially, both items are similar (light circles), and diversity is low. However, $u_1$ and $u_2$ incentivize $x_1$ and $x_2$, respectfully, to move away from each other, results in a more diverse set for $u_0$ (in this case, with no loss in accuracy).}
	\label{fig:illust}
\end{figure*}

%-----------------------------------------------------------------


\subsection{Strategic content creators}
Our key modeling assumption is that items are owned by strategic \emph{content creators}
(or `suppliers') whose aim is to maximize exposure to their items \citep{hron2022modeling}.
Content owners act to increase their item's score $s(x_j)$,
which is an average over the scores of potentially relevant users: % $i \in U_j$:
% we model the system as revealing minimal and equitable information regarding scores
\begin{equation}
s(x_j) = \avg \{f(x_j;u_i) \mid i \in U_j\}
\end{equation}
To preserve equity across content creators,
we use spherical averaging over user representations $u_i$ to maintain unit norm\footnote{To see why normalizing $v$ is important here, consider an item $j$ with two users: if $u_1,u_2$ are close, then $v_j$ will have a similar norm, but if $u_1,u_2$ are spread out, $\|v_j\|$ can be significantly smaller.}, which reduces to the following form: %\looseness=-1
\[
% f(x_j;\vtilde_j) =
s(x_j) = 
\vtilde_j^\top x_j,
\,\,\text{ where }\,
\vtilde_j = \frac{v_j}{\|v_j\|}, \,
v_j = \frac{1}{m_j} \sum_{i \in U_j} u_i %f_i(x_j)
% , \qquad \vtilde_j = \frac{v_j}{\|v_j\|}
\]
This can be taken to mean that the system reveals normalized scores,
so that utility for item $j$ derives from $\vtilde_j$
which describes an `average' user
representing all $i \in U_j$.

Following the general formalism of strategic classification \citep{hardt2016strategic}, we assume content creators can modify their item's features, at a cost, and in response to the learned predictive model.
Given a cost function $c(x,x')$,
content creators modify items via the \emph{best response} mapping:\footnote{We adopt the standard convention and assume $c$ is fixed, uniform across content creators, and known to all.}
\begin{equation}
\label{eq:best_response}
\Delta_f(x_j) = \argmax_{x':\|x'\| = 1} \,
% f(x';\vtilde_j) 
s(x_j)
- \alpha c(x_j, x') % \,\,\, \text{s.t.} \,\,\, ||x'||_2 = 1	
\end{equation}
where the norm constraint ensures that modified items $x^f_j = \Delta_f(x_j)$
remain on the unit sphere,
and 
throughout we consider quadratic costs,
$c(x,x') = \|x-x'\|_2^2$.\extended{\footnote{As in \citet{levanon2021strategic,levanon2022generalized,jagadeesan2022supply,eilat2022strategic}.}}
The scaling parameter $\alpha \ge 0$ will allow us to vary the intensity of strategic updates:
when $\alpha$ is small, modifications are less restrictive
and so $x^f_j$ can move further away from $x_j$, and vice versa.\looseness=-1

We consider item modification to be `real', in the sense that changing $x$
can cause $y$ to also change.
Following \citet{shavit2019extracting, rosenfeld2020predictions},
we assume labels are determined by an unknown
ground-truth function $f^*$
which determines personalized relevance for any counterfactual item $x$ as $y=f^*(x;u^*_i)$,
where $\{u^*_i\}_{i=1}^m$ are ground-truth user preferences
(which are unknown to the learner).
This can be relaxed to assuming a fixed conditional $p^*(y|x;u_i^*)$.

\paragraph{Strategic behavior and diversity.}
Eq. \eqref{eq:best_response} reveals how the system can drive incentives: since each content creator $j$ acts to make their item more aligned with $\vtilde_j$, the system can set the $u_i$
(which together compose all $\vtilde_j$) to induce $\vtilde_j$-s that vary in their orientation;
this incentivizes different content creators to move towards different directions---thus creating diversity,
whose potential growth rate is mediated by $\alpha$.
Note that even linear $f$ can incentive different items to move in different directions, since
(i) due to norm constraints, items will not necessarily move in the direction of the gradient of $f$;
and (ii) more importantly, since different items appeal to different users,
each $\vtilde_j$ defines a utility function $s(x_j)= f(x_j;\vtilde_j)$
that is distinct for item $j$.
% different content creators can be incentivized to move their items in different directions.
% This is for two reasons:
% First, due to norm constraints, items will not necessarily move in the direction of the gradient of $f$; even for a fixed $f$, different $\alpha$ can entail different directions for $\smash{x^f_j}$, since it must lie on the unit sphere.
% Second, and more importantly, items have different incentives because they gain utility
% from different groups of users, which is expressed by each item having a different $\vtilde_j$.
Nonetheless, the $\vtilde_j$ are not disjoint;
the connectivity structure in $G$ forms dependencies across the $u_i$,
which introduce correlations in how 
% induce a dependency structure that defines how
items can jointly move
(see Fig. \ref{fig:illust} (B)).


% \blue{Figure \ref{fig:user_embd} shows the best response of item creator in a different cost factors $\alpha$.}
% \nir{say here that different content creators move in different directions, and explain why. otherwise the linear model may create the (wrong) impression that all points move in the same direction and distance. consider having $v$ explicitly depend on $x$.}
% \nir{say changing $\alpha$ affects distance from $x$, and that norm constraints mean $x'$ changes in orientation, not magnitude}

\extended{
\paragraph{Label updates.}
Contrary to vanilla strategic classification,
we allow changes in item features $x$ to trigger changes
in corresponding relevance scores $y$.
This is in line with works on causal strategic learning,
in which modifications to $x$ can causally affect outcomes
downstream.
For concreteness,
and similarly to \citet{shavit2019extracting, rosenfeld2020predictions},
we assume labels are determined by an unknown
ground-truth function $f^*$
which determines personalized relevance for any counterfactual item $x$ as $y=f^*(x;u^*_i)$,
where $\{u^*_i\}_{i=1}^m$ are ground-truth user preferences
(which are unknown to the learner).
From a modeling perspective,
relying on $f^*$ for determining counterfactual outcomes
is useful since it makes our problem one of \emph{covariate shift} \citep{bickel2009discriminative},
for which retraining is a sound approach.
Note $f^*$ can be quite distinct from $f$ (e.g., can be non-linear), and in our experiments we take several measures
to differentiate them.}

%-----------------------------------------------------------------



\subsection{Interaction dynamics}
\label{subsec:dynamics}
We will be interested in studying how learning affects ranking accuracy 
and diversity over time.
As noted, we focus on retraining dynamics,
where at each round $t$ the system re-trains its predictive model
on data gathered at the previous round $t-1$.
The goal of retraining is to update the model to be accurate on current data,
which may have changed since the model was last trained;
in our setting, such changes are due to strategic item modifications.
We think of item modification as a process which takes time:
% initially,
in the initial portion of the round,
users remain to observe the previous $\smash{x_j^{(t-1)}}$;
only later, and after some time has passed,
the updated $\smash{x_j^{(t)}}$ are revealed,
and users provide updated relevance ratings $\smash{y_{ij}^{(t)}}$.
This justifies the system's choice to train on the current
unmodified $\smash{x_j^{(t-1)}}$ (i.e., \emph{before} distribution shift),
as well as the need to periodically re-train its predictive model
on the modified $\smash{x_j^{(t)}}$ with fresh labels $y_{ij}^{(t)}$
(i.e., \emph{after} the shift).
% This will allow us to contrast \emph{reactive} 
% learning strategies with \emph{proactive} strategies that anticipate change.


\extended{
We model interactions between the learning system, strategic content creators, and users as follows.
Interactions occur over time and in discrete rounds,
where each round $t$ includes three steps:
(i) At the beginning of the round,
the system uses data collected in the previous round %, $S^{(t-1)}$,
to learn current user representations $\smash{u_i^{(t)}}$,
which it then uses for recommendations $\smash{\r_i^{(t)}}$;
(ii) During the round, content creators respond to the system
by strategically modifying their corresponding items $\smash{x_j^{(t)} \mapsto x_j^{(t+1)}}$;
(iii) Finally, towards the end of the round,
% (and after modifications have taken place),
users consume recommended items and report relevance ratings $\smash{y_{ij}^{(t)}}$ for the updated $\smash{x_j^{(t)}}$,
% We next describe in detail the different aspects of this interaction.
which are then used as input for the system in the 
next round.
% \[
% S^{(t)}	= \{ (u_i^{(t)}, x_j^{(t)}, y_{ij}^{(t)})\}_{ij}
% \]
}

% Broadly, our dynamic model aims to capture a certain form of temporal distribution shift, caused performatively by the system through its effect on strategic behavior.
% but also update its learned model according the modified $\smash{x_j^{(t)}}$ (after distribution shift).
% (before distribution shift),
% but also account for the future effects of the modified $\smash{x_j^{(t)}}$ (after distribution shift).

% We next describe each step of the interaction process in detail.

% https://tex.stackexchange.com/questions/5191/how-to-raise-a-subscript

% \paragraph{Learning objective.}
% The primary goal of the system is to recommend relevant items.
% Here we consider the conventional ranking metric of NDCG, evaluated on the top $k$ items.
% Consider a list of $K$ items with relevance scores $\y=(y_1,\dots, y_K)$.
% Let $\r=(r_1,\dots,r_K)$ be a ranking, and
% denote by $\r(\ell)$ the index of the $\ell^{\text{th}}$-ranked item in $\r$.
% Then the top-$k$ discounted cumulative gain (DCG) is defined as:
% \begin{equation}
% \label{eq:DCG@k}
% \DCGk(\y, \r) = \sum_{\ell=1}^k\frac{2^{y_{\r(\ell)}}-1}{\log(1+\ell)}
% % \DCGk(\y, \r) = \sum_{\ell=1}^K \1{r_\ell \le k} \frac{2^{y_\ell}-1}{\log(1+r_\ell)} 
% \end{equation}
% % \nir{itay: make sure this is correct.}
% where $2^{y_j}-1$ measures the `gain' in relevance from having item $j=r(\ell)$ in the top $k$, and $\log(1+\ell)$ `discounts' its rank.
% NDCG is then obtained by normalizing relative to the optimal ranking
% $\r^* = \argmax_{\r} \DCGk(\y,\r)$.
% % $\r^*$:
% %  as $\NDCGk(\y, \r) = \DCGk(\y, \r) / \DCGk(\y, \r^*)$.
% % \begin{equation}
% % \label{eq:NDCG@k}
% % \NDCG(\y, \r) = \frac{\DCGk(\y, \r)}{\DCGk(\y,\r^*)}
% % \end{equation}
% % % where $r^* = \argmax_{r'} \DCGk(r',y)$
% % We consider score-based ranking, where items are ranked
% % by a personalized score function $f_i(x)=f(x;u_i)$:
% % via:
% % \begin{equation}
% % \r_i = \rank(f(x_1;u_i),\dots,f(x_K;u_i))
% % \end{equation}
% The goal of the system is therefore to learn
% %score functions $f_{u_i}$, parameterize by
% user representations $u_i$
% that optimize average NDCG on the top-$k$ items:
% \begin{equation}
% \max_{u_1,\dots,u_m} \frac{1}{m} \sum_{i=1}^m
% \NDCGk(\y_i,\r_i)
% \end{equation}
% where $\r_i = \rank(f(X_i;u_i))$ is the ranking of items in $X_i$ for user $i$.
% For learning, we will assume that the system has access to relevance labels
% $y_{ij}$ for a subset of user-item pairs $(i,j) \in E$,
% and the goal is to generalize well to other pairs.


% Following \citet{hron2022modeling, jagadeesan2022supply}\tocitec{others?},
% we consider linear score functions $f(u,x) = u^\top x$,
% which are sufficiently expressive for our purposes \citep{ferrari2019we}.
% Linear scores are used extensively in the strategic learning literature
% since the learned $u$ can be interpreted as estimated user preferences
% (as in Expected Utility Theory \tocite),
% and since they permit tractable strategic responses \tocitec{strategic regression papers with linear predictors}. %\footnote{Despite using linear scores,  responses in our setting are \emph{not} linear due to graph dependencies and normalizing constraints.}
% For learning, we will assume that the system has access to relevance labels
% $y_{ij}$ for a subset of user-item pairs $(i,j) \in E$,
% and the goal is to generalize well to all pairs.



% Our platform contains $m$ users and $n$ items. Each item has $d$ features.
% \nir{who has $d$ features - users? items? both?} \itay{Items. We changed the setting. users don't have features only items. The RS learn representation of users in the item space (the embedding.}
% Each user $i$ is assigned with $l$ items that might be relevant to him. Those items are considered his recommendation list, and they are denoted by $X_i$.
% \nir{are we thinking of this as queries and results that need to be ranked? or as the output of a `first-stage' ranker in two-stage recommendation (see Joachims paper)? or both?} \itay{I think we can see it as both. It is the output of the first stage (which find relevant items to user. In the second stage we rank items in $X_i$. We can think about the user as a query (note that there are no features to the user as I said above)}.
% \nir{At some point should say this give bipartite graph - decide when and where this makes most sense} \itay{Yes, but I am not sure where and I hope it won't create confusion.}
% Item $x_a$ might be in the recommendation list of more than one user. We denote the set of users that the item $x_a$ is in their recommendation list in $U_{x_a}$. For example if item $x_a$ is in the recommendation list of users $i$ and $j$  $x_a \in X_i$, $x_a \in X_j$ and $i, j \in U_{x_a}$. We can represent the recommendation lists of all users as Bipartite graph which his two vertex group are the users and the items. Each edge $(i, x_j)$ in the graph represents that item $x_j$ is in the recommendation list of user $i$.  
% The main goal of the RS is to order the items according to their relevance to the user. One of the most common evaluative measures to evaluate ranking order is Normalized Discounted Cumulative Gain (NDCG). 
% Given set of items and their relevance to the user: $\{y_i\}_{i=1}^l$ and some order $r$ of the items: $r = (r_1, r_2, ..., r_l)$ where $r_i \ne r_j \quad \forall i \ne j$ and $r_i\in [1, l]$.
% The Discounted Cumulative Gain (DCG) is defined as follows:\\
% \begin{equation}
% \DCG(r, y)@k = \sum_{i=1}^k\frac{2^{y_{r_i}}-1}{\log(1+i)}
% \label{DCG_r}
% \end{equation}
% A vector $y$ represents the relevance of items in a list and an entry $i$ represents the relevance of item $i$. $k \le l$ is the last position in the list to be calculated for DCG. Note that the enumerator encodes item relevance (``gain''),
% which the denominator penalizes (``discounts'') according to the item's rank. 


% \todo{Figure \ref{fig:user_embd} (left)}

% \subsection{Regularization for creating diversity}

% Let $\similar(x_1, x_2)$ be some pairwise item similarity metric (e.g., cosine similarity), and define the corresponding distance measure by $d(x_1, x_2)=1 - \similar(x_1, x_2)$.
% A common measure of the diversity of items
% within a set is Intra-List Diversity (ILD) that used in \citet{ziegler2005improving, antikacioglu2019new, vargas2011rank} which penalizes \red{diversity/similarity(?)} according to all pairwise distances (normalized).
% However, most of the time this metric takes into account only the top $k$ items in the list (\red{cite?}). Thus given items list in order $r$, DIV for user $i$ is defined as follows:
% \nir{i think it's more intuitive to use the notation $\mathrm{DIV}(\cdot)$, rather than ILD (even if it's more `correct)}
% % \begin{equation}
% \begin{align*}
% &DIV_i(X_i;r)@k =  \\
% & \frac{\sum_{x_t, x_j \in X_i}^l x_t \cdot \1{r_t \le k} \cdot x_j \cdot \1{r_j \le k}d(x_t, x_j)}{1/2\cdot k(k-1)}
% % & \frac{2}{k(k-1)}\sum_{x_t, x_j \in X_i}^l x_t \cdot \1{r_t \le k} \cdot x_j \cdot \1{r_j \le k}d(x_t, x_j)
% \end{align*}
% % \end{equation}

% We can average for all users in the system and define objective for optimize the average intra-list diversity for all users:
% \begin{equation}
% DIV(X, U) = -\frac{\sum_{i = 1}^m DIV_i(X_i; r^i)}{m}
% \label{DIV_obj}
% \end{equation}
% \nir{what is the range of values of ILD? $[0,1]$?} \itay{Yes. But it is not practically to get 1 (unlike NDCG) when the recommendation list is in length higher than 2.}
% Here X is a tensor in shape $(m, l, d)$ and $r^i$ denotes the order of items in the recommendation list for user $i$. 
% Our RS has two goals: The main goal to achieve high NDCG and the second goal is to achieve high diversity. Unfortunately achieving both of them many time is not feasible. Consequently we purpose to control the trade off of accuracy diversity with regularization parameter that determines the importance of the diversity. We can now formalize the learning objective includes our regularization:
% \begin{equation}
% \argmin_{U \in R^{m \times d}} \frac{1}{m} \sum_{i=1}^m L(u_i,X_i,y_i) + \lambda \cdot DIV(X, U) 
% \label{non_st_objective}
% \end{equation}
% \nir{if i understand correctly, this seems to present what we refer to as the `non-strategic baselines' as *our* method. we should carefully think of how to present this, and when to start talking about time} \itay{I agree I wasn't sure if to insert the non strategic in this section. I thought to show it only as baseline in the real data experiment. But I thought it might be nice to show figure \ref{fig:user_embd} which explains how the model control the ranking by changing the user embedding}
% Note that the RS control the embedding of each user and by changing it direction it can control the importance of the diversity. Figure \ref{fig:user_embd} (left) demonstrate how the system changes user embedding to control NDCG and to control of DIV. The figure also demonstrate the trade off between those two. 



% - exposure-maximizing content creators
% - producers compete for a finite user attention pool by crafting content ranked highly by a given algorithm



% \subsection{Item diversity}
% In addition to ranking accuracy,
% we will also be interested in measuring and promoting diversity across recommended items. Here we focus on intra-list diversity
% \citep{ziegler2005improving,vargas2011rank,antikacioglu2019new}
% and use cosine similarity as a metric,
% % $\cos(x,x') = x^\top x' / \|x\|\|x'\|$
% $\cos(x,x') = \frac{x^\top x'}{\|x\|\|x'\|}$
% which is appropriate for comparing unit-norm features
% \citep{ekstrand2014user, hron2022modeling}.\footnote{Since features are normalized, we have $\cos(x,x') = x^\top x'$.}
% For a list of items $X$ and ranking $\r$,
% diversity for the top-$k$ items is defined as:
% \begin{equation}
% \label{eq:divk}
% \divk(X,\r) = 
% % \diversity(X,\r) = 
% \frac{1}{k(k-1)}
% \sum_{j,\ell=1}^k 1-\cos(x_{\r(j)},x_{\r(\ell)})
% \end{equation}
% % We will use Eq. \eqref{eq:diversity} to meausre diversity, and explictly optimize it.
% which takes values in $[0,1]$ \citep{smyth2001similarity}.


% Since item features vary over time and as a result of strategic updates,
% we can expect strategic behavior to be a driving force in determining
% eventual diversity across items;
% and since items are updated to increase their scores,
% in learning $f$, the system holds potential power to shape incentives and steer
% towards diverse outcomes.
% Key to this is the fact that content creators differ in their utility,
% i.e., have different $\vtilde_j$---which the system controls.
% The challenge is that diversity may trade off with NDCG
% (see Fig. \ref{fig:illust} (A)).
% Before discussing how this can be used to promote diversity in Sec. \toref,
% we 


% \red{
	% - [consider moving to end of section] \\
	% - how we expect diversity to arise from strategic behavior \\
	% - sphere constraints \\
	% - initial diversity in 1st stage \\
	% - different $v_j$ for each content creator
% }


\extended{
\subsection{Relation to performative prediction}
- performative
  -- retraining
  -- stateful!
- what changes (x and y!), D operator
  -- same population, so no actual `distribution' to change
- time scales
  -- `even' and `odd' times
  -- 1st stage recs (=lists) do not change
- `constraint': want ndcg to be good *now*
- strategic updates take time; want to have good div *later*, before next retraining
- pre/post: definition, meaning


Note that unlike other works in which utility derives from a linear predictive model
\tocitec{strat reg, strat ranking; others?},
in our setting different items move in different manners.
This is since:
(i) items must remain on the unit sphere
(which also implies that cost budgets do not necessarily deplete), and
(ii) utility is personalized per item (due to different user sets $U_j$).
As we will show, the latter point is crucial for creating diversity.
}

%============================================================

% \subsection{Strategic behaviour of content creators}
% Content creator are willing to maximize their profit. In order to achieve this they would like to get a better score from the recommended system on the users that are in the recommendation list (i.e all the users that the product is in their recommendation system). Those users might have a little different taste in some features and it is not possible to find a change that is satisfy all of them. As a result item producer wish to change the item features in a way that gets maximum score on the average of the embedding of the users in $U_{x}$. Our setting assumes that when item improves in one features it has to come over another feature. We find this assumption realistic since in the real world it is not possible to improve all features to maximum value since the resource are limited and improve on one aspect might harm other. Therefore we normalized every item feature vector to 1 and constrained the item movement to keep item norm as 1 (which has been done in \citet{hron2022modeling}).
% \nir{need to ground this by citing another paper that does this. pretty sure the jordan paper does; try to find others that do too!}
% Modifying the item comes with a cost that is is determined by a function $c:  \R^d \times  \R^d \rightarrow \R$. Content creator will modify his product if the cost it pays for the change is lower than the improvement in the score (similar to \citet{tsirtsis2019optimal, jagadeesan2022supply}). We can now write the content creator’s best-response update:
% \begin{equation} \label{eq:best_response}
% \Delta(x) = \argmax_{x' \in \X} \,\, 
% v^Tx' - \alpha c(x', x) \quad s.t \quad ||x'||_2 = 1
% \end{equation}
% \red{note: this is *not* budget, because of sphere constraints. $\alpha$ determines how far you can move on the sphere, ie, the length of the arc}
% % \nir{this is of course the tricky part where we need to argue why content creators (i) optimize their *scores*, and not actual rankings, and (ii) do not account for the strategic actions of other creators}
% Where $\alpha$ is a scalar that balanced between the improvement of the items and the cost content creator pays for the change.  
% $v$ is the normalized embedding average of the users in $U_x$ i,e: \red{explain about the normalization why do we need it.}
% \begin{equation}
% v = \frac{v'}{|v'|}\quad  v' = \frac{1}{|U_x|}\sum_{i \in U_x}\frac{u_i}{|u_i|}
% \label{avg_u}    
% \end{equation}
% \red{note: items move wrt *all* items, not only top k! think carefully how to motivate this. }
% The item creator wants to treat each user in $U_x$ equally. In the absence of normalizing the users' embedding vectors, users with higher magnitudes would have a greater influence on vectors (which inequality). We normalize the vector $v$ to be a unit vector since the average of the user embedding only influences the optimal direction for changing the item. If the item $x$ is not normalized, its ability to change depends on the magnitude of the vector $v$ rather than just its direction.       
% \nir{give xeplicit formula for it}
% The changes that item might effect the diversification.
% This mathematics formulation has a closed-form solution when $c(x', x)= ||x'-x||_2^2$ (As shown in appendix \ref{apx:best_response}): 
% \begin{equation} \label{eq:best_response_close}
% \Delta(x) = \frac{v+2\alpha x}{|v+2\alpha x|}
% \end{equation}
% Figure \ref{fig:user_embd} shows the best response of item creator in a different cost factors $\alpha$.
% \nir{say here that different content creators move in different directions, and explain why. otherwise the linear model may create the (wrong) impression that all points move in the same direction and distance. consider having $v$ explicitly depend on $x$.}

% \nir{don't we have justified reasons for our choices of item features and/or user embedding that have to do with `fairness' or equity (for users? content creators? both?) if this is still true - state them where relevant.} \itay{Ok it is written in orange.}


==> synthetic_exp_plots/macro.tex <==


% Recommended, but optional, packages for figures and better typesetting:
\usepackage{verbatim}
\usepackage{microtype}
\usepackage{subfigure}
\usepackage{enumitem}
\usepackage{booktabs} % for professional tables
\usepackage{color,graphicx}
\usepackage{comment}
\usepackage{thmtools, thm-restate}
\usepackage{hyperref,xcolor}
% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2021} with \usepackage[nohyperref]{icml2021} above.
\usepackage{hyperref}
\usepackage{amssymb,amsmath,amsthm,dsfont,bm,mathtools, bbm}
\usepackage{xfrac}
\usepackage[bottom]{footmisc}

\newcommand{\red}[1]{} %{{\leavevmode\color{red}{#1}}}
\newcommand{\blue}[1]{} %{{\leavevmode\color{blue}{#1}}}
\newcommand{\green}[1]{} %{{\leavevmode\color[RGB]{0,128,0}{#1}}}
\newcommand{\purple}[1]{} %{{\leavevmode\color[RGB]{128,0,255}{#1}}}
\newcommand{\orange}[1]{} %{} %{{\leavevmode\color[RGB]{229,83,0}{#1}}}
\newcommand{\lblue}[1]{{\leavevmode\color[RGB]{0,128,255}{#1}}}
\newcommand{\darkgray}[1]{{\leavevmode\color[RGB]{140,140,140}{#1}}}
\newcommand\todo[1]{{\red{TODO: {#1}}}}
\newcommand\tocite{\red{[CITE]}}
\newcommand\tocitec[1]{\red{[CITE: {#1}]}}
\newcommand\toref{\red{[REF]}}
\newcommand\torefc[1]{\red{[REF: {#1}]}}
\newcommand\extended[1]{{\orange{EXTENDED: {#1}}}}
\newcommand{\nir}[1]{\green{[NIR: {#1}]}}
\newcommand{\itay}[1]{\purple{[ITAY: {#1}]}}
\newcommand{\niradd}[1]{\green{{#1}}}
\newcommand{\naive}{{na\"ive}}
\newcommand{\Naive}{{Na\"ive}}

\newcommand\expect[2]{\mathbb{E}_{#1}{\left[ {#2} \right]}}
\newcommand\prob[2]{\mathbb{P}_{#1}{\left[ {#2} \right]}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\softmax}{softmax}
\DeclareMathOperator{\topk}{topk}
\DeclareMathOperator{\rev}{rev}
\DeclareMathOperator{\sort}{SORT}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\key}{KEY}
\DeclareMathOperator{\avg}{avg}
\DeclareMathOperator{\similar}{sim}
\DeclareMathOperator{\diversity}{div}
\newcommand{\divk}{{\mathrm{div}_{@k}}}
\DeclareMathOperator*{\relevance}{relevance}
\DeclareMathOperator*{\score}{score}
\newcommand{\DCG}{{\ensuremath{\mathrm{DCG}}}}
\newcommand{\NDCG}{{\ensuremath{\mathrm{NDCG}}}}
\newcommand{\DCGk}{\ensuremath{\mathrm{DCG}_{@k}}}
\newcommand{\NDCGk}{\ensuremath{\mathrm{NDCG}_{@k}}}

\newcommand{\NNDCGk}{\text{NNDCG}{@k}}
\newcommand{\NDCGsoft}{{\text{NDCG}_{\text{soft}}}}
\newcommand{\ILD}{{\texttt{ILD}}}
\newcommand{\DIV}{{\texttt{DIV}}}
\newcommand{\sig}{{\texttt{sig}}}
\newcommand{\AGG}{{\texttt{AGG}}}
\newcommand{\intra}{{\texttt{Intra-list term }}}
\newcommand{\ndcgterm}{{\texttt{NDCG term }}}
\newcommand{\method}[1]{{\fontfamily{lmtt}\selectfont{{#1}}}} %{{\textsc{{#1}}}}

\newcommand{\1}[1]{\mathds{1}{\{{#1}\}}}
\newcommand{\one}[1]{\mathds{1}_{\{{#1}\}}}

% \newtheorem{assumption}{Assumption}
\newcommand{\X}{{\cal{X}}}
\newcommand{\calH}{{\cal{H}}}
\newcommand{\calHhat}{{\hat{\cal{H}}}}
\newcommand{\x}{{\bm{x}}}
\renewcommand{\r}{{\bm{r}}}
\newcommand{\rhat}{{\hat{\r}}}
\newcommand{\y}{{\bm{y}}}
\newcommand{\Y}{{\cal{Y}}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\br}{{\Delta}}
\newcommand{\brapx}{{\hat{\Delta}}}
\newcommand{\fapx}{{\hat{f}}}
\newcommand{\Fapx}{{\hat{F}}}
\newcommand{\yhat}{{\hat{y}}}
\newcommand{\vtilde}{{\tilde{v}}}
\newcommand{\utilde}{{\tilde{u}}}
\newcommand{\Phat}{{\hat{P}}}

\newcommand{\iid}{{\stackrel{_{\text{iid}}}{\sim}}}
\newcommand{\cg}{{\texttt{cg}}}

\newcommand{\err}{{\mathtt{err}}}
\newcommand{\fstar}{{f^{\star}}}
\newcommand{\fhat}{{\widehat{f}}}
\newcommand{\pr}{{\mathbb{P}}}


\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}



==> synthetic_exp_plots/method.tex <==
\section{Learning and Optimization}
\label{sec:Learning}

% - regularizing for diversity
% - lookahead regularization
% - differntiable ndcg; P, soft ranks
% - differentiable div
% - anticpating responses; differentiable Delta
% - time: learn one step, interested in acumulative effects over time


The conventional approach for learning to recommend
relies on training predictive models to correctly rank
items by their relevance. % (e.g., using NDCG).
% \blue{When done in retraining, this amounts to RRM algo studied in performative prediction.}
Then, to promote diversity,
a post-hoc procedure is typically used to re-rank
$\r$,
% , e.g., by traversing the list and removing items
% similar to those in higher positions \citep{carbonell1998use}.
which in our setting can affect diversity by determining which items appear in the top $k$. %, over which $\diversity$ is computed.

The main drawback of re-ranking is that its heuristic nature
means that diversifying the list might reduce its relevance,
and can cause NDCG to deteriorate substantially.
% and therefore provides no guarantees on the resulting NDCG,
% which may deteriorate substantially.
As an alternative, here we pursue a more disciplined approach,
in which we directly optimize the joint objective:
\begin{equation}
\label{eq:learning_objective_non-strat}
\max_{u_1,\dots,u_m} \frac{1}{m} \sum_{i=1}^m \NDCGk(\y_i,\r_i) + 
% \frac{\lambda}{m} \sum_{i=1}^m \diversity(X_i,\r_i)
\lambda \, \divk(X_i,\r_i)
\end{equation}
where $\r_i = \rank(f(X_i;u_i))$ is the ranking of items in $X_i$ for user $i$,
and $\lambda$ trades off between accuracy and diversity.
Thus, by considering $\diversity$ as a regularizer,
we can tune $\lambda$ to obtain a desired balance.
In our experiments we tune $\lambda$ to achieve a predetermined level of NDCG (e.g., 0.9); in this case, regularization serves as a criterion for choosing the most diverse model out of all sufficiently-accurate models.
% can be interpreted as a criterion for choosing of all models $f$ which obtain this level of accuracy the one which is most diverse.

We next describe our approach for optimizing
Eq. \eqref{eq:learning_objective_non-strat},
which sets the ground for our strategically-aware objective.


\subsection{Optimization}
% \todo{make it clear what is our contribution and what is not. emphasize strategic part more, elaborate on why it's non-trivial}
We propose to optimize Eq. \eqref{eq:learning_objective_non-strat}
by constructing a differentiable proxy objective,
to which we can then apply gradient methods.
The key challenge is that Eq. \eqref{eq:learning_objective_non-strat} relies on a ranking operator (i.e., for computing NDCG and top-$k$),
which is non-differentiable.
Our approach adopts and extends \citet{Pobrotyn2021NeuralNDCGDO},
and makes use of the differentiable sorting operator introduced in \citet{grover2018stochastic}.
First, consider NDCG.
For the numerator, note that the ranking operator $\r(\cdot)$ can be implemented
using a corresponding permutation matrix $P$, i.e., 
$y_{\r(\ell)} = (Py)_\ell$. % when ranking $y$. %, and similarly for $X$.
To differentiate through $\r$, we replace $P$ with a `smooth'
row-wise softmax permutation matrix,
$\Phat$. %, defined as:
% \nir{what is the softmax over?}
We denote by $\rhat$ the corresponding soft ranking,
computed as 
$\rhat = (\Phat \odot Q)^\top \bm{1}$,
where $Q_{ij} = i \,\,\forall j$, $\odot$ is the Hadamard product,
and $\bm{1}$ is a vector of 1-s.
The denominator for $\NDCGk$ requires accessing indexes in $y$ using explicit entries in $\r$;
applying $\rhat$ instead gives a weighted combination of $y$-s, with most mass concentrated at the correct $\r(\ell)$ when $\rhat$ is a good approximation.
The summation term is implemented using a soft top-$k$ operator,
which we obtain by applying an element-wise scalar sigmoid to $\r$ as:
\begin{equation}
\1{r \le k} \approx \sigma_{\tau}(k-\rhat)    
\end{equation}
For the diversity term, note that $\cos$ is naturally differentiable.
To make the entire $\divk$ differentiable,
we use the soft top-$k$ operator on item pairs via:
% to obtain a smooth regularizer:
\begin{equation}
\frac{1}{k(k-1)} \sum_{j,j'}^n
\sigma_\tau(k-\rhat_j) \sigma_\tau(k-\rhat_{j'})
\left(1 - x_j^\top x_{j'}\right)
\end{equation}

% $\sum_{j,\ell=1}^k 1-\cos(x^f_{\rhat(j)},x^f_{\rhat(\ell)})$



% \green{
% \begin{equation}
% \Phat_{j\cdot} = \softmax _\tau(f(x_j;u))
% \end{equation}
% where $\tau$ is a temperature parameter.
% }


\subsection{Strategically-aware learning}
Although Eq. \eqref{eq:learning_objective_non-strat} accounts for diversity in learning, it does so \emph{reactively}, in a way that is tailored to the previous time step.
Since the learned $f$ incentivizes content creators to modify items,
we propose to promote diversity \emph{proactively} by anticipating their strategic responses.
To do this, we replace $X_i$ with the anticipated
$X^f_i =  \Delta_f(X_i) = \{\Delta_f(x)\}_{x \in X_i}$
% in $\diversity$
to get our strategically-aware objective:
\begin{equation}
\label{eq:learning_objective_strat}
\max_{u_1,\dots,u_m} \frac{1}{m} \sum_{i=1}^m \NDCGk(\y_i,\r_i) + 
% \frac{\lambda}{m} \sum_{i=1}^m \diversity(X_i,\r_i)
\lambda \, \divk(X^f_i,\r^f_i) %\\
% & \text{where} \quad
% X'_i = \Delta_f(X_i), \,\,\,
% \r'_i = \rank(f(X'_i;u_i))
\end{equation}
where $\r^f_i = \rank(f(X^f_i;u_i))$ is the anticipated ranking.
Eq. \eqref{eq:learning_objective_strat} optimizes for pre-modification NDCG,
but promotes post-modification diversity; this is the mechanism through which
learning can incentivize the creation of diversity.\footnote{While in principle it may be possible to also consider future NDCG,
note this necessitates reasoning about how deploying $f$ affects future $y$, which is a challenging causal inference task.}
\extended{with $\diversity$ now serving as a `lookahead' regularizer
that anticipates outcomes in the next time step.}
% Although diversity is considered only one step ahead,
% we expect it to preserve---and even improve---over time.
% towards the \emph{creation} of a diverse collection of items.
% with $\alpha$ affecting its growth rate.


The challenge in optimizing Eq. \eqref{eq:learning_objective_strat} is
twofold: (i) $\Delta_f$ is an argmax operator, which can be non-differentiable,
and (ii) $\Delta_f$ depends on $f$ both internally (by determining utility)
and externally (in the top-$k$ operator of $\divk$).
Fortunately, for our modeling choices,
$\Delta_f$ can be solved in a differentiable closed form.
Using KKT conditions, we can derive:
\begin{equation} \label{eq:Delta_closed_form}
\Delta_f(x_j) = \frac{\vtilde_j + 2\alpha x_j}{|\vtilde_j + 2\alpha x_j|}
\end{equation}
Proof in Appendix \ref{apx:best_response}.
Plugging Eq. \eqref{eq:Delta_closed_form}
into Eq. \eqref{eq:learning_objective_strat}
gives us our final, differential strategic learning objective.


% \todo{Fig. \ref{fig:user_embd}(\textbf{right})}

% - system can incentivize strategic behavior by controlling $u$-s
%   - \ref{fig:user_embd}(\textbf{right})
% - operationalize by encoding strategic response in div()
% - closed form Delta; differentiable
% - expect this to *create* diversity
% - as lookahead step \citep{rosenfeld2020predictions}
%   - can do this for div since it only uses x' and does not need y' (ndcg does!)
% - expect div to accumulate over time; relation to alpha

% \red{
    % - goal: optimize ndcg now, diversity later \\
    % - affects of $\alpha$ on rate of diversity growth \\
    % - ndcg now as a "constraint", diversity later as a means to create diversity (rather than "force" it)
% }

% \blue{
% This mathematics formulation has a closed-form solution when $c(x', x)= ||x'-x||_2^2$ (As shown in appendix \ref{apx:best_response}): 
% \begin{equation} \label{eq:best_response_close}
% \Delta(x) = \frac{v+2\alpha x}{|v+2\alpha x|}
% \end{equation}
% }

%===============================================================

% \subsection{Exploiting strategic movement for diversification}

% \red{closed form $\Delta$}

% Since the items changes are caused by the users embedding that the RS creates, RS can strategically create user embedding that will cause strategic changes that increase the diversity. To achieve this the learning objective should simulate the strategic response of content creator i.e the items after the modification ($\Delta(x)$). We follow \citet{eilat2022strategic} and include the item after the modification in the learning objective. Note that changing in item usually takes time. Thus, while the RS creates recommendation list the items hasn't perform the change. The primary goal of RS it to provide items order according to current relevance to the user. Hence, item should be able to provide high NDCG before strategic changes and provide high diversity after the strategic changes have been done. We adjust the learning objective in equation \eqref{non_st_objective} to include the strategic response in the diversity regularization. This change create look-ahead regularization (similarly to \citet{rosenfeld2020predictions}) that balance between accurate sorting in current time to diversity in the future: 
% \begin{equation}
% \label{strategic obj}
% \argmin_{U \in R^{m \times d}} \frac{1}{m} \sum_{i=1}^m L(u_i,X_i,y_i) + \lambda \cdot DIV(\Delta(X), U) 
% \end{equation}
% After the strategic change has been done items should be more diverse and it should be easier to build recommendation list that is both diverse and accurate. In order to ensure diversity for long period, it might necessary to continue use the diversity look-ahead regularization which prevents diversity to decrease. In some setting when $\alpha$ is high the item producer has to pay high cost for each change. The diversity increases a little at a time, so to create a high diversity, it is necessary to use regularization over a long period of time and test it after several time stamps. The result is a periodic structure in which RS publishes user embeddings and items producers change their features in response to those embeddings. For accurate predictions, the RS must collect interactions with items after the change and retrain itself. There is no anticipate about the ndcg after the changes since the RS doesn't have the relevance of items after the content creator preform the modification. It takes time to the RS to collect new data and meanwhile the system is less accurate. This repeated two stages structure has become recently very common in many works that study agent classifier model interaction \citep{perdomo2020performative}.  
% % Content creator are willing to change their products in order to achieve better score on the classifiers in some cost. Content creator are familiar with their audience thus they know their embedding. 
% \nir{goal: optimize ndcg now, diversity later; ndcg now as a "constraint", diversity later as a means to create diversity (rather than "force" it)}

% \nir{say we will be interested in effects that accumulate over multiple time steps. consider connecting this to the literature on performative prediction.}
% The RS is aware of the structure of the bipartite graph that indicates which item is in the recommendation list of each user. Since RS control the user embedding it might be able to change those embedding to incentive content creator to change their products in a way that increases the diversity. A demonstration of this ability is described in \ref{fig:user_embd}(\textbf{right}).


% \blue{
% The order of items can also be defined using a permutation matrix. You can reorder numbers in range 1 to $l$ by multiplying the vector $[1, l]$ (all the integers between 1 and $l$) by matrix permutation $P$. The following is an alternative definition of DCG:\\
% \begin{equation}
% \DCG(P, y)@k = \sum_{i=1}^k\frac{2^{(Py)_i}-1}{\log(1+i)}
% \label{DCG_P}
% \end{equation}
% $(py)_i$ is the entry $i$ in the vector $py$
% }
% %  $\NDCG$ is obtained by normalizing w.r.t. the optimal ranking, $P^*$:
% % \begin{equation}
% % \NDCG(P,y)@k = \frac{\DCG(P,y)}{\DCG(P^*,y)}, 
% % P^* = \argmax_{P'} \DCG(P',y)
% % \end{equation}
% % Since the relevance of items to user is not given the RS, Many RS tries to learn for each user i a vector embedding $u_i \in \R^d$ that represents the importance of each feature to the user. One of the most common way to rank items in set of items according to their relevance to user is by dot product between user embedding and each item features \citep{hron2022modeling, jagadeesan2022supply}. The higher the product $u_i^Tx_j$ the higher the score of item $x_j$ and it will be placed higher in the recommendation list. Therefore, the RS uses embeddings as a decision rule when ranking items and tries to find the embeddings with the highest NDCG. In order to learn the optimal user preference the RS collects previous interactions between users and items i.e $\{x_i, y_i\}_{i=1}^l$. $x_i \in \R^d$ denotes the item feature and $y_i \in \R$ is item relevance to the user.
% \blue{
% Since permutation matrix can present any order of items it also can represent order resulting from a user's preferences vector. Thus, the matrix $P$ in equation \eqref{DCG_P} is function of the user embedding. The system look for each user i the vector $u_i$ that maximize this measure. If we stack all the users embedding vector to one matrix $U \in R^{d \times m}$, we can define the learning objective: 
% \begin{align}
% &\argmin_{U \in R^{d \times m}} \frac{1}{m}\sum_{i=1}^m L(u_i,X_i,y_i), \\
% &L(u_i,X_i,y_i) = - \NDCG(\hat{P}(u_i,X_i), y_u)
% \end{align}
% Where $\hat{P}$ is a matrix permutation that sorts the items in $X_i$ by the following rule: $u_i^Tx$. Thus $\hat{P}$ is function of $u_i$ and $X_i$.
% }

% \blue{
% Note that $r$ can be achieved by multiplication every row $j \in [1, l]$ in matrix $P$ by the integer $j$ and then summing each column. This computation can be written explicitly:
% \begin{equation}
%     r = (P*Q)^T 1_v
% \label{raking_from_p}
% \end{equation}
% Here $1_v$ is a vector that contains only ones, $Q$ is matrix that the column i contains i and $*$ is the element wise product (Hadamard product).
% Therefore $r$ is function of $u_i$ and $X_i$.
% }

% \subsection{Optimization for NDCG}
% For getting high NDCG we have to find an optimal users embedding using optimization methods like \citet{duchi2011adaptive, DBLP:journals/corr/KingmaB14}. However, those methods requires differentiable objective function which NDCG is not. To obtain a differentiable proxy for NDCG, we adopt the approach of \citet{Pobrotyn2021NeuralNDCGDO}
% who propose a differentiable NDCG-based loss for neural architectures.
% The key element is a smooth sorting operator, introduced in \citet{grover2018stochastic}
% and implemented as a row-wise softmax permutation matrix operator,
% $\hat{P}$. Our proxy loss will be based on this `soft' NDCG metric which means replacing $P$ in equation \eqref{DCG_P} by $\hat{P}(\tau)_{\NDCG}$. Note that the temperature parameter $\tau$ of the softmax influences the smoothness of the matrix which means smaller $\tau$ a better approximation.

% \subsection{Optimization for diversity}


% Since the regularization is operated on the items after the strategic response $\Delta(x)$, We calculated new matrix permutation$\hat{P}(\tau)_{\DIV}$ that approx the sorting according to the relevance of items after the strategic movement i.e $u_i^T\Delta(x)$ instead of $u_i^Tx$. As we mentioned vector $r$ that define the ranking in equation \eqref{DIV_obj} can be calculated by matrix $\hat{P}(\tau)_{\DIV}$ If we use in the approximation $\hat{P}(\tau)_{\DIV}$ instead of $P'$ we get soft rank vector
% $r_{\tau_\DIV}$. Now we can use the soft rank vector for replacing the indicator $\1{r_j \le k}$ in equation \eqref{DIV_obj} by differential operator. We use the sigmoid  function to approx this 1-0 indicator in the following way:
% \begin{equation}
% \1{r_j \le k}^{soft} = \sigma_{\tau_{\sig}}(k-r_{\tau_{\DIV}})
% \end{equation}
% Note that the $\tau$ that used for NDCG DIV and sigmoid might be different.  
% \nir{need to say that we can optimize future div because we can anticipate modified features $x'$, but can't optimize future ndcg because for that we need to predict $y'$, which we can't} \itay{That true but I explain it in different way. I said that the main goal of RS is to find relevance items. That should be at the present while diversity might take time to be created. Nobody wants will use RS that will recommend items that be relevance in the future}

% \begin{figure}[h]
%   \includegraphics[width=\linewidth]{strategic_response.pdf}
%   \caption{Item creator's best response. The original item features are marked as x. The ideal vector for changing an item to is v. However, best response depends on \red{cost factor} $\alpha$. By lowering $\alpha$, we see that the item's best response becomes closer to v.}
%   \label{nonstrategic_demonstration}
% \end{figure}


% This mathematics formulation has a closed-form solution when $c(x', x)= ||x'-x||_2^2$ (As shown in appendix \ref{apx:best_response}): 
% \begin{equation} \label{eq:best_response_close}
% \Delta(x) = \frac{v+2\alpha x}{|v+2\alpha x|}
% \end{equation}


==> synthetic_exp_plots/real_data_exp.tex <==
\section{Experiments on Real Data}
\label{sec:real data}
In this section we evaluate our approach on real data,
and study how NDCG and diversity evolve over time under different
learning methods and experimental conditions.
See ther Appendix 
for additional details (\ref{apx:Data details}) and results (\ref{apx:results_real}).\looseness=-1

% Additional results can be found in Appendix \ref{apx:results_real}.

\paragraph{Data.}
Our experimental setup is based on the restaurants portion of the Yelp dataset\footnote{\url{https://www.yelp.com/dataset/download}},
which includes user-submitted restaurant reviews.
We focus on users having at least 100 reviewed restaurants.
For each user $i$, we construct the list of potential items $X_i$
to include the 40 most popular restaurants of those reviewed by $i$,
% chosen to maximize cross-user overlap
% (i.e., maximize the number of edges in the graph).
which amounts to 236 users and 1,520 restaurants in total.
% Further details in Appendix \ref{apx: recommendation list creation}.
We elicit $d=43$ restaurant features
(e.g., cuisine type, noise level)
to be used by the system for learning.
We also elicit `ground truth' user features $u^*_i$
used for optimizing $f^*(x',u^*_i)$,
which is trained to predict the likelihood that $i$ will review $x$,
interpreted here as relevance $y$.
The labeling function $f^*$ is used only for determining
update relevancies $y$ for modified items $x'$;
neither $f^*$ nor the $u^*_i$ are known to the learner.
% and are used only for determining ground-true labels
% as follows.
% % Further details are given in Appendix \ref{apx:Data details}.
% To determine how changes in $x$ affect relevancies $y$,
We ensure $f^*$ is distinct from learnable functions $f$ by several means:
(i) $f^*$ is a fully-connected deep network, whereas $f$ are linear;
(ii) $f^*$ is trained using true user features $u^*_i$, which are unobserved for $f$;
(iii) $f^*$ is trained on considerably more data,
of which the data used for training $f$ is a non-representative subset;
and
(iv) $f$ is trained on labels that are modified to emphasize highly-rated items.
Full details in Appendix \ref{apx:training f^*}


\paragraph{Setup and learning.}
We consider top-10 recommendation (i.e., $k=10$),
% so that the goal of the system is to recommend the top-10 relevant items (out of 40).
and evaluate performance over $T=10$ rounds of retraining and corresponding strategic updates.
For training, 
we assume that at each round the system has access to 30 items per user,
randomly selected (out of the 40) per round;
of these, a random 20 are used for training, and the remaining 10 for validation
(tuning $\lambda$ and early stopping).
Test performance is evaluated on all 40 items.
Since the test set includes additional items (compared to training),
$f$ must learn to generalize well to new content at each step.
Since adding items also changes the graph,
and since the graph determines strategic responses---$f$ must also learn to generalize to new forms of strategic updates.

\paragraph{Methods and evaluation.}
In line with our dynamic model (Sec. \ref{subsec:dynamics}),
all methods we consider are aimed primarily at optimizing `current' NDCG,
i.e., at time $t$ optimize NDCG on $x^{(t)}$.
The methods we consider differ in how (and if) they promote diversity, and include:
(i) a \method{non-strategic} approach which regularizes for current diversity on non-strategic inputs $x^{(t)}$ (Eq. \eqref{eq:learning_objective_non-strat}),
(ii) our \method{strategic} approach, which regularizes for future diversity on the anticipated $x^{(t+1)} = x^{f_t}$ (Eq. \eqref{eq:learning_objective_strat}),
(iii) an accuracy-only \method{baseline}, which does not actively promote diversity
(by setting $\lambda = 0$),
(vi) the baseline approach, augmented with the popular \method{MMR} re-ranking procedure for diversification \citep{carbonell1998use},
and (v)
a hybrid approach in which we apply \emph{strategic} for $t=5$ rounds and then `turn off' regularization.
% which mimics \method{baseline} for the remaining rounds.\looseness=-1

Since \method{non-strategic} and \method{strategic} are designed to balance NDCG and diversity,
for a meaningful comparison,
in each experimental condition we fix a predetermined target value for NDCG,
tune each method to achieve this target at each round,
and compare the resulting diversity.
Technically, this is done by tuning $\lambda$ (up to tolerance 0.01) on the validation set.
We use the notation $\lambda_{\beta}$ to mean that $\lambda$
was tuned for the target $\beta$.
% (e.g., $\lambda_{0.9}$ for NDCG=$0.9$).
To compare with \method{baseline}, in one condition we set $\lambda$ to the largest value that maintains the same NDCG as the baseline (for which $\lambda=0$),
denoted $\lambda_{\text{base}}$.\looseness=-1
% (post-hoc analysis shows that this achieves stable and near-target values in all conditions).
% For the constrained methods we use NDCG=0.85,0.9,0.95, and NDCG=1, which is comparable to the no-regularization baseline.

Finally, note that due to performativity, data at time $t$ depends on the learned model at time $t-1$. Because our dynamics are \emph{stateful}, results are path-dependent,
and so comparisons must be made across full trajectories---and cannot be made independently at each time point.


%=====================================================================
\begin{figure}[b!]
    \centering
    \includegraphics[width=\columnwidth]{real_data_plots/ndcg_div_high3_5.pdf}
    \caption{
    Pareto curves for \method{strategic} per round (varying $\lambda$; solid lines), and vs. \method{baseline}.
    Dashed lines show per-$\lambda$ trajectories.\looseness=-1
    % Pareto curves for \method{strategic} over rounds, and in comparison to \method{baseline}. Solid lines depict variation across $\lambda$, and dashed line show per-$\lambda$ trajectories.
    }
    \label{fig:tradeoff}
\end{figure}
%=====================================================================    

    

\subsection{Diversity over time}
Our first experiment studies how diversity evolves over time
for different NDCG targets.
Fig.~\ref{fig:experiements_real} (left) shows diversity (top) and NDCG (bottom) per round
for $\alpha=0.1$, which permits significant (yet restricted) strategic updates.
Results show that for \method{baseline}, which does not actively promote diversity,
average diversity decreases over time by roughly 40\%.
Adding \method{MMR}, which re-ranks for diversity, improves only marginally.
In the $\lambda_\text{base}$ condition,
diversity for \method{non-strategic} improves only slightly
compared to \method{baseline}, mostly at the onset.
In contrast, our \method{strategic} approach is able to consistently maintain (and even slightly increase) diversity over time,
albeit at small occasional drops in test NDCG, as compared to \method{non-strategic} ($\le 0.02$).\footnote{One possible reason for \method{baseline} to achieve NDCG$\approx$1 is that when diversity is extremely low,
items are so similar (and hence similarly relevant) that choosing the top-k
becomes trivial.}
In the $\lambda_{0.9}$ condition, \method{non-strategic} is able to preserve roughly 80\% of diversity by sacrificing $\sim 13\%$ of the optimal NDCG.
Meanwhile, and for the same loss in NDCG,
\method{strategic} is able to quickly \emph{double} the initial diversity---and sustain it, likely through means similar to those observed in Sec. \ref{sec:synth_vary_costs}.
Note that sustaining diversity requires to actively promote it throughout; once regularization is switched off, diversity immediately drops.%\looseness=-1

Fig. \ref{fig:experiements_real} (center) shows results for a similar setting, but using a larger $\alpha=2$.
In comparison, here diversity for all methods improves---but for \method{baseline} and \method{MMR}, this is only transient.
Results are also smoother, and accumulate---for both improvement and deterioration, which is likely due to the fact that strategic movements are now more restricted.
The biggest distinction here is that for $\lambda_{0.9}$, \method{non-strategic} eventually obtains the same level of diversity as \method{strategic}, where the advantage of 
\method{strategic} is that it improves much faster.
This is also likely due to $\alpha$ being large:
small updates mean that $x$ and $x^f$ are correlated,
and so regularizing for $\diversity(X,\r)$
also improves $\diversity(X^f,\r^f)$ to some extent.

\subsection{The role of modification costs.}
To further examine the role of $\alpha$,
we compare performance across a range of cost scales
and for multiple target NDCG values.
Fig. \ref{fig:experiements_real} (right) shows
diversity at $T=10$.
As can be seen, all methods benefit from increasing $\alpha$.
However, diversity for \method{baseline} remains below 
that of a \method{random} baseline which recommends $k$ random items.
For \method{strategic}, sacrificing fairly little NDCG ($\lambda_{0.95}$ and below) suffices for gaining significant diversity across \emph{all} $\alpha$.
Results also show how $\alpha$ mediates the gap between \method{non-strategic} and \method{strategic}, which increases as $\alpha$ grows.\footnote{To avoid clutter we plot \method{non-strategic} only for $\lambda_{0.9}$, which is comparable to Fig. \ref{fig:experiements_real} (left) and (center), but note that other target NDCG values exhibit qualitatively similar patterns.}\looseness=-1

\subsection{Tradeoffs over time.}
To understand how NDCG and diversity trade off,
Fig. \ref{fig:tradeoff} shows the Pareto curves,
obtained by varying $\lambda$, for \method{strategic}
and over several rounds.
Results show that the entire curve improves over time;
paths within each target NDCG condition shows specific trajectories, which are in line with the choice of the chosen target value.
Comparison to the trajectory of \method{baseline}
shows that even when accuracy is (approximately) maximized,
the system still holds a certain degree of freedom in choosing $f$, which it can use to steer content creators towards a more diverse collection of items, with the benefit of newly-created diversity becoming more significant over time.




\extended{
\todo{add pre/post update results}

Recall that our dynamic setup (Sec. \toref) assumes that updates
occur over time.
At each step $t$ we report the performance
on the current data $x^{(t)}$
of the previous model $f^{(t-1)}$ (trained on $x^{(t-1)}$) and the current-trained model $f^{(t)}$ (trained on $x^{(t)}$).

Since we model strategic updates as taking place over time,
intuitively we would expect that performance for $f^{(t-1)}$ degrade from $t-1$ to $t$, but due to accuracy constraints, that all post-training accuracies will be the same. This lets us focus on how diversity evolves.

- when retraining, points don't move; only reason div changes is because top-k set can change (otherwise, div would be the same!) \\
- note retraining for lookahead improves div; in principle, objective was supposed to optimize div before retraining (and after movement); but retraining can help if $x'$ and $x''$ are correlated \\

}

% first consider ndcg=1:
% - without directly optimizing diversity, it goes down (non-reg baseline)
% - optimizing for diversity now slightly improves diversity now, but costs in terms of ndcg, and the effect goes away in the next time step; worse, over time, div is as low as without regularization
% - when we optimize regularization for later (lookahead), diversity increases, and over time - kept fairly stable. ndcg is lower than w/o regularization, but on par with reg for now.

% for ndcg=0.9 - which we think of as willingly giving up ndcg for div:
% - reg for now still cannot improve div over time, despite `giving up' ndcg. drop in ndcg within rounds is considerable.
% - however, optimizing for ndcg later (lookahead) now increases diversity substantially; ndcg is again on par with reg for div now.

% - when retraining, points don't move; only reason div changes is because top-k set can change (otherwise, div would be the same!) \\
% - note retraining for lookahead improves div; in principle, objective was supposed to optimize div before retraining (and after movement); but retraining can help if $x'$ and $x''$ are correlated \\
% - ndcg can be if div is so low so that order doesn't matter, because relevancies are nearly the same. (for $\lambda=0$, ndcg start $<1$ and grows, and div decreases)

% \red{
% time-dependence within trajectories - where?
% }


%===============================================================
% \green{\rule{\columnwidth}{3pt}}

% \paragraph{Experiment setting:}
% We now evaluate our model on a real dataset Yelp\footnote{\url{https://www.yelp.com/}}. 
% Yelp is a website that allows user to share reviews about businesses they have encountered. The website publish dataset which documented for each user his past business interaction. Thus we could construct for each user his items in the recommendation list. To narrow our RS we focus only in business that are consider as restaurant.
% According to our setting the RS tries to suggest user to restaurant it might be interested to visit. Therefore, we look for past interaction of user and business ignoring the reviews this user has assign \red{should we admit it?? but if not the reviews might ask why we didn't use the rank user gave to business}. The dataset includes basic character to each restaurant such as price, location, noise level type of food (i,e Burgers, vegan, Japanese, Italian) and more other features. We used 43 features. the full feature list and more information about the data can be find in \ref{apx:Data details}.\\
% Our experiment includes interactions between users and restaurants after strategic modification has been performed, so we must simulate the relevance of the restaurant to the user ($y'$). Similarly to \citet{shavit2019extracting, rosenfeld2020predictions} we determine $y$ by a model that assign score in $\R$ to each user and item $f^*(\overrightarrow{u}, x)$. The score indicates how likely it is that a user will visit the restaurant. The relevance of item to user ($y$) is calculated by using $f^*$ in the following way:
% \begin{align*}
%     y = 2^{f^*(\overrightarrow{u}, x)}
% \end{align*}
% To increase the penalty in NDCG when items are ranked incorrectly, we use an exponent function.
% As opposed to the RS model which infers user vector preferences, the ground truth model $f^*$ requires user features (which according to our settings are hidden to the RS model) to assign score to each pair of items and users. More information about  $f^*$ training and $\overrightarrow{u}$  can be found at \ref{apx:training f^*}.\\
% We restricted the data to users with more than 100 reviews to avoid users with few interactions.
% Each user was given a 40-item recommendation list based on their previous interactions. Please refer to \ref{apx: recommendation list creation} for a detailed explanation of how we choose those 40 items for each user.
% We measured top-10 diversity for all datasets. \\
% Our goal in this experiment is to test our model over time and see how it affects diversity over time. Our assumption is that RS are willing to maximize diversity of recommendation lists, but there is a limit to their willingness to sacrifice NDCG. As hyper parameters, we consider this NDCG limitation. RS tries to get maximum diversity when NDCG on the test set is within some threshold of NDCG limit. The threshold was set to 0.1 In this experiment we compare different RS with different NDCG limit.
% RS exposes partial information about the items, and there may be additional items that have yet to be anticipated. In the future, after the system has completed training, those items will be added to the system. Hence, the RS must be capable of generalizing to achieve high NDCG on recommendation lists that include new items. For each user, we assume that the RS knows 30 restaurants out of 40. Each time the RS trains a user, we randomly select 30 restaurants to make sure the RS is familiar with them. A new 10 items will be added to the 30 during test time. RS selects 20 of 30 restaurants to be included in the train set randomly in order to produce generalization. Adding the other 10 restaurants to the 20 serves as a simulation for new items and together the 30 restaurants serve as a validation set. Validation sets are used to determine $\lambda$ and the number of epochs the model is training on.
% In line search for $\lambda$ values between 0 and 100 we look for the model with the highest diversity in the range that is allowed using NDCG.
% \blue{\paragraph{Diversity over the time.} In our problem setting, training occurs every two time stamps, while items' features change every two time stamps. Each model that trains at even time $t$ is tested on the test set at the same time and on the data after strategic response to the model at time $t+1$.}
% As baselines, we consider models that trained without regularization (i.e. $\lambda = 0$) and models that use regularization without strategic modification, i.e. equation \eqref{non_st_objective} instead of \eqref{strategic obj}.
% Twenty time stamps were used for the experiment (training has been done only at even times).
% You can find the results at figure \ref{fig:real data time}. We let the items change with a low limitation \red{$\alpha=0.1$}. It is evident that ignoring diversity leads to a decrease in diversity, whereas models taking diversity into account produce a higher diversity. A model that achieves high diversity without taking strategic behavior into account, i.e. regularization at the current time, sometimes suffers from very low diversity after strategic modifications. Diversity significantly decreases after one time stamp, going below the average diversity at time 0 (the gray dotted line in). 
% As a contrast, the model with lookahead regularization incorporates strategic changes in order to create diversity over time. The model gets high diversity when it is willing to compromise on NDCG, and the diversity remains high over time. By looking at the NDCG, we can see that the feature changes harm the NDCG in all models. Restaurants with high budgets may change their features drastically, affecting the distribution the RS observed during training. However, when using no regularization ($\lambda = 0$) or small regularization that archives high NDCG, the RS tends to learn user preference better, which leads to incentive changes that maximize y. \red{should we explain that the random base line increase as well or show utility graph??}.
% \red{Important: explain the sharp decrease better and say we can't prevent them. Those decreases happens when there is strategic movement and cite preformative prediction papers.} \\
% \paragraph{NDCG diversity trade off}.
% The NDCG diversity trade-off is now viewed from a different perspective. In figure \ref{fig:real data ndcg div}\textbf{left}, we show NDCG diversity in the 4 first time stamps with cost factor $\alpha=2.0$ (small budget). There is a trade-off between NDCG diversity in each graph. Each graph loses NDCG as diversity increases. Both kinds of regularization and this small budget increase diversity when the strategic modification is made. However, the regularization that considers the next step exploits the strategic modification better and reaches a higher level of diversity. The NDCG diversity trade off exists also at low values of $\alpha$, as shown in \red{appendix}.
% \paragraph{The influence of modification budget ($\alpha$).}
% Our experiment examines the effect of the modification budget on diversity after many time stamps (19). The diversity decreases below the initial diversity (gray dotted line) without regularization. The diversity is higher for lower NDCG target values, as expected (similar to the NDCG diversity experiment we described previously). Our analysis in section \ref{sec:analysis} noted that when item changes are less sharp, i.e not tremendous changes, it is easier for the model to control the diversity and achieve better diversity after enough training item response iterations. For all curves, we observe in figure \ref{fig:real data ndcg div} (right) that the higher $\alpha$, the smaller the ability to change restaurant features and the greater the diversity.         

% \caption{\textbf{Left - NDCG diversity trade off:} The blue and red curve represent the NDCG diversity curve that created by the model that anticipate the strategic movement. The blue lines are the result on test set after the training (before the strategic movement) while the red curve are the results after the strategic movement. Similarly, the orange and the green curves are the results of the model with regularization $\Delta(x)$. The light curves represents the next iteration of training and strategic modification. \textbf{right - The influence of the budget limitation $\alpha$:} The diversity in the last time stamp as function of $\alpha$.  }





       


      

==> synthetic_exp_plots/related.tex <==

\subsection{Related work}
\label{sec:related}

% \red{TODO: add papers on: \\
% - how recommendations lack diversity \\
% - how diversity decreases over time \\
% - important measures in recsys beyond accuracy (eg, diversity, serendipity, coverage) \\
% - motivation papers
% }

\extended{
\todo{read and add: Diversified Recommendations for Agents with
Adaptive Preferences / neurips 2022}}


\paragraph{Diversity in recommendation.}
The literature on diversity in recommendation is extensive; here we present a relevant subset.
Early approaches propose to diversify via re-ranking
\citep{carbonell1998use, bradley2001improving, ziegler2005improving},
an approach that remains to be in widespread use today
\citep{abdollahpouri2019managing}.
More recent methods include 
diversifying via functional optimization \citep{zhang2008avoiding}
or integration within matrix factorization \citep{su2013set, hurley2013personalised,cheng2017learning}.
Diversity has also been studied in
sequential \citep{kim2019sequential}
and conversational \citep{fu2021popcorn}
settings.
% To the best of our knowledge, none of these methods
% consider strategic behavior.
%
The idea of using regularization to promote secondary objectives
in recommendation has been applied for
controlling popularity bias \citep{abdollahpouri2017controlling},
enhancing neutrality \citep{kamishima2014correcting},
and promoting equal opportunity \citep{zhu2021popularity}.
% Closest in spirit to ours is 
For diversity,
\citet{wasilewski2016incorporating} apply regularization,
but assume that the system has direct control over (latent) item features;
this is crucially distinct from our setting in which
the system can only indirectly encourage content creators to apply changes.
% , indirectly through the learned scoring rule.


% Diversification of the recommendation system has been an important consideration throughout the years, resulting in many methods being developed to enhance it. Traditional methods for intra-list diversification date back to \citet{carbonell1998use, bradley2001improving, ziegler2005improving}, which propose a greedy re-ranking procedure for balancing relevance and diversity based on pair-wise item similarities.
% Later approaches propose do diversify by solving appropriate optimization problems
% \citep[e.g.,][]{zhang2008avoiding}.
% Other works integrate intra-list diversity measures into matrix factorization-based collaborative filtering methods \citep{su2013set, hurley2013personalised}
% or optimize diversity-promoting supervised learning objectives end-to-end \citet{10.1145/3038912.3052585}.
% Recent works propose novel neural architectures for this task. For example, \citet{sun2020framework} introduced a Bayesian graph convolutions neural network that models the uncertainty in user-item relation, and utilize this to enhance diversity. Nevertheless, none of these studies addressed the strategic behavior of content producers, which we will see in the next sections may greatly influence diversity.


\paragraph{Strategic learning.}
There has been much recent interest in studying learning in the presence of
strategic behavior.
\citet{hardt2016strategic} propose \emph{strategic classification} as a framework
for studying classification tasks in which users (who are the targets of prediction) can modify their features---at a cost---to obtain favorable predictions.
This is based on earlier formulations by
\citet{bruckner2009nash,bruckner2012static},
with recent works extending the framework to settings in which users act on noisy \citep{jagadeesan2021alternative}
or missing information \cite{ghalme2021strategic,bechavod2022information},
have broader interests \citep{levanon2022generalized},
or are connected by a graph \citep{eilat2022strategic}.
Since we model content creators as responding to a scoring rule,
our work pertains to the subliterature on \emph{strategic regression},
in which user utility derives from a continuous function
\citep{rosenfeld2020predictions,tang2021linear,harris2021stateful,bechavod2022information},
and strategic behavior is often assumed to also affect outcomes
\citep{shavit2020causal,harris2022strategic}.
Within this field, our framework is unique in that it considers content creators---rather than end-users---as the focal strategic entities.
The main distinction is that this requires learning to account for the \emph{joint} behavior of all strategic agents (rather than each individually),
which even for linear score functions results in complex behavioral patters 
(c.f. standard settings in which linearity implies uniform movement \citep{liu2022strategic}).




\extended{For example, 
\citet{rosenfeld2020predictions} and \citet{levanon2021strategic} also use regularization to drive secondary objectives,
but in setting that are unrelated to recommendation,
and in which user responses fully decompose.}

% and particularly on causal stratgic regrssion
% since we permit strategic feature update to also affect item relevance,
% our work also draws connections to the literature on causal strategic learning
% \tocitep{}

% Most works in strategic learning consider linear score functions
% since they permit tractable user responses,
% as do we here.
% However, whereas in other works linearity simplistically implies
% that all features `move' in the same way
% (this is key in e.g. \citet{liu2022strategic},
% who study strategic score-based ranking),
% our recommendation setting introduces a dependency structure which breaks this notion of uniformity.
% Our work also permits changes in features to causally affect outcomes

% Recently, the strategic behavior resulting from the classifier has attracted a great deal of attention and many studies have been conducted in this area. One of the most poplar study is \citet{hardt2016strategic}. According to this setting, agents manipulate their features to get positive predictions while learners look for rules that are robust to those changes. Many works adopted this setting (or a similar setting with a few extensions) and some assumed that the agent intended to get positive classification \citep{levanon2021strategic, pmlr-v162-levanon22a, pmlr-v139-ghalme21a, jagadeesan2021alternative, estornell2021unfairness, eilat2022strategic}, while others assumed it intended to improve continuous scoring \citep{tang2021linear, bechavod2022information}. Those works assumed that changes in the agent's prediction did not change his labeling.
% Several works assumed, however, that the features modification was not superficial, but also reflected in the true label \citep{rosenfeld2020predictions} \red{add more}. Part of them, like our work,  design decision rules that encourage agents to take actions that further a goal the strategic agent didn't necessarily intend to pursue \citep{tsirtsis2019optimal, kleinberg2020classifiers}. 
% In our case the agents are directed in a way that increase diversity.
% In our case the agents try to maximize their score in the RS but we direct them to change their feature in a way that increases diversity. 


% \paragraph{Strategic behavior in recommendation.}
\paragraph{Performativity and incentives.}
% Performative prediction % \citep{perdomo2020performative}
% is a useful framework for reasoning about how learned predictive models affect the environment in which they operate.
The current literature on performative learning focuses primarily on macro-level analysis,
such as providing sufficient global conditions for retraining to converge
\citep{perdomo2020performative,miller2021outside,brown2022performative}
or proposing general optimization algorithms
\citep{mendler2020stochastic,izzo2021learn,drusvyatskiy2022stochastic,maheshwari2022zeroth}.
In contrast, performativity in our setting emerges from micro-level modeling of strategic agents in a dynamic recommendation environment,
and our goal is to address the specific challenges inherent in our focal learning task.
Within recommendation,
content creators (or `supplier') incentives 
have also been studied from a game-theoretic perspective 
\citep{ben2018game,Ben-Porat_Goren_Rosenberg_Tennenholtz_2019,ben2020content,jagadeesan2022supply,hron2022modeling}.
Here, focus tends to be on notions of equilibrium,
and the system is typically assumed to have direct control over outcomes
(e.g., determining allocations or monetary rewards).
Our work focuses primarily on learning,
and studies indirect incentivization through a learned predictive rule.

\extended{
Finally, we note that in terms of experimentation,
virtually all works that study behavior in recommendation---as does ours---rely on simulation for evaluation
\citep[e.g.,][]{jiang2019degenerate,sun2019debiasing,zhan2021towards,kalimeris2021preference,yao2021measuring},
and in particular for retraining \citep{krauth2020offline}.
Recommendation is at its core a policy problem;
hence, appropriate evaluation requires means for measuring counterfactual outcomes
(i.e., what ``would have happened'' under a different recommendation)---for which simulation has been advocated as a primary candidate
\citep{ie2019recsim,chaney2021recommendation,curmei2022towards}.
% In our work we use simulation as well, but make efforts to tie it to real data
}


% \red{TODO: detail more on each paper}
% A number of papers have examined the relationship between RS and strategic behavior by studying the contest between content creators and examining the equilibrium \citep{Ben-Porat_Goren_Rosenberg_Tennenholtz_2019, pmlr-v151-liu22b, jagadeesan2022supply, hron2022modeling}.
% All of the above improve some criterion after the modification, but \citet{rosenfeld2020predictions} suggested a regularization that balanced prediction accuracy before and improvement after the modification. We use similar framework but in our work the modification of each agent is dependent on the other as we present in section 2


% There were works that involve ranking and recommendation system with strategic behaviour.  Most of those works study the contest between different different product and the character of equilibrium \citep{ben2019recommendation, pmlr-v151-liu22b, jagadeesan2022supply, hron2022modeling}. Although some of those paper create decision rule that incntive content creator to equilibrium with some properties that relevant to the RS, Our work is different since we present RS that explicitly achieve diversity after the strategic changes.   


% Most of those study adopted the setup of \citet{hardt2016strategic}. In this setting agents try to get positive prediction according decision rule by manipulate their features. Many works adopted this setting  
% Those strategic modification might cause prediction errors. according some classifier by manipulate strategically their features with out actually change their true label.       


% \todo{
% - strategic regression\\
% - performative prediction\\
% - kurland+tenenholtz\\
% - jordan papers
% }


% - papers on diversity in recommendation (but no strategic behavior) \\
% - differentiable ranking \\
% - strategic classification (and regression!); say we allow change in y \\
% - performative prediction - maybe? \\
% - strategic ranking - models dependencies, but no actual learning \\
% - other papers on incentives in recsys (eg jordan paper, maybe one of omer's papers, kurland+tenenholtz) ***
% - paper about strategic behavior in recommendation that also mention/talk about diversity (?) \\
% - lookahead



==> synthetic_exp_plots/synthetic.tex <==
% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=0.4\textwidth]{synthetic_exp_plots/div_changes.pdf} \qquad
%   \includegraphics[width=0.4\textwidth]{synthetic_exp_plots/ndcg_changes.pdf}
%   \caption{diversity \textbf{(Left)} and ndcg \textbf{(Right)} vs number of switches between different users.}
%   \label{user_ovelap}
%   \end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.32\textwidth]{synthetic_exp_plots/div_up_ndcg_down_changes.pdf}
\includegraphics[width=0.32\textwidth]{synthetic_exp_plots/div_up_ndcg_down_stdu.pdf} 
\includegraphics[width=0.32\textwidth]{synthetic_exp_plots/varying_cost_lam1000.pdf} 
\caption{
\textbf{Experiments on synthetic data.}
\textbf{(Left)} Diversity and NDCG for increasing overlap between users and for multiple $\lambda$. As more edges are swapped (and overlap increases), diversity quickly peeks. For higher $\lambda$,
significant diversity is obtained even with minimal overlap.
\textbf{(Center)} Diversity and NDCG for increasingly dispersed true user preferences ($u^*$). Without regularization, diversity is minimal even for highly varied preferences ($\sigma_{u^*}=1$).
With regularization, even if mild, diversity increases dramatically, albeit with some loss in NDCG.
\textbf{(Right)} Diversity and NDCG for varying cost scales $\alpha$ under large $\lambda$.
For low modification costs ($\alpha=1$), learning is unable to incentivize diversification.
But this changes sharply once $\alpha \ge 1$,
with larger $\alpha$ requiring more time for diversity to 
smoothly form.
}
\label{fig:synth}
\end{figure*}

\extended{
\begin{figure}[b!]
\centering
\includegraphics[width=0.9\columnwidth]{synthetic_exp_plots/angle dispersion 3.pdf}
\caption{
Dispersal of items $x_i \in \R^2$ over time.
}
\label{fig:angles}
\end{figure}
}

\section{Synthetic Experiments}
\label{sec:synthetic}
Our previous section showed that,
under favorable conditions,
it is theoretically possible 
to generate significant diversity through incentivization.
In this section we show that diversification is also empirically possible 
by applying our strategically-aware learning approach
(Eq. \eqref{eq:learning_objective_strat})
to a series of increasingly-complex synthetic tasks.
Each task is designed to explore the role of a different factor in our setup,
and to shed light on how accuracy and diversity trade off as $\lambda$ is varied.
Additional results can be found in Appendix \ref{apx:additional_result}.

% intended to gradually move from the simplified setting of Sec. \ref{sec:analysis} to the full setting considered in \ref{sec:real data}.
% under different experimental conditions.
% - diversity in item user groups
% - diversity in true user preferences
% - over time
% - modification costs $\alpha$
% [complement theory + move beyond gradually move from simplified setting of previous section to our full setting, studied empirically on real data in the next section.]
% [Focus on our approach (sec 2).
% In particular, here we will consider how diversity trades-off with accuracy, by varying $\lambda$.]

\paragraph{Experimental setup.}
We set $n=200,m=50,k=K_i=10$ for all $i$,
and fix $d=2$ so that features $x,u$ can be easily visualized as angles.
% \nir{what is $k$?} \itay{$k=K_i=10$}
Item features $x$ are sampled from
$\mathcal{N}((\sfrac{1}{\sqrt{2}},\sfrac{1}{\sqrt{2}}),\sigma^2_x I)$.
We use $f^*(x;u_i^*) = 2^{(u_i^*)^\top x}$,
where ground truth user preferences $u^*$
are sampled from
$\mathcal{N}((\sfrac{1}{\sqrt{2}},\sfrac{1}{\sqrt{2}}),\sigma^2_{u^*} I)$.
All features are normalized post-sampling.
We use $\sigma_x=1$ and $\sigma_{u^*}=0.1$,
but in some settings vary them to control dispersion.
% \nir{or is it always stdev=1 for items?} \itay{in cost modification exp it is less. I wanted to show how that diversity may increase.}
% \blue{Item lists for users were generated by sampling items uniformly without replacement, which ensured (w.h.p.) some diversity across $U_j$.}
All results are averaged over 100 random repetitions (when applicable).
Further details and additional results in Appendix \ref{apx:additional_result}.

% \todo{go over experiment details table}

% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=0.4\textwidth]{synthetic_exp_plots/div_stdu.pdf} \qquad
%   \includegraphics[width=0.4\textwidth]{synthetic_exp_plots/ndcg_stdu.pdf}
%   \caption{\textbf{(Left)} diversity vs user standard deviation. \textbf{(Right)} ndcg vs user standard deviation.}
%   \label{std_div}
% \end{figure*}


%------------------------
\subsection{The role of variation in user item lists}
We begin by investigating the importance of variation across user item lists,
which complements and extends our results in Sec. \ref{sec:diversity_strategic_incentives}.
To vary the degree of overlap, we start by partitioning users and items into five distinct groups and drawing edges between all group members;
this creates five sub-graphs---mutually-exclusive across,
and fully-overlapping within.
Then, for each experimental condition $N \in \mathbb{N}$,
we form links across sub-graphs
by randomly `shuffling' $N$ edges, in a way which preserves node degrees.
As $N$ increases, density within components grows,
and between them shrinks;
as a result, overlap is reduced.
For large enough $N$, each pair $(i,j)$ has (approximately) equal probability of being linked, resulting in little overlap.
\extended{\todo{find reference for this method!}}
% Here we set $\sigma_{u^*}$ to a fairly low value of 0.1.

Figure \ref{fig:synth} (left) shows NDCG (before strategic updates; bottom) and diversity
(after strategic updates; top) for increasing $N$ and for a range of $\lambda$.
For $N=0$ (full overlap), diversity is zero for all $\lambda$,
in line with Prop. \ref{prop:Full_users_overlap}.
As $N$ increases, diversity also grows, but at the cost of reduced NDCG, which is more pronounced for larger $\lambda$.
Note how only minimal overlap (e.g., $N=100$ for $\lambda=1$) suffices for generating considerable diversity, which rises sharply once $N>0$.
This suggests our approach can utilize the capacity for diversity implied by Prop. \ref{prop:diff_users_max_div},
% even under accuracy constraints.
even under accuracy constraints.\looseness=-1


% - connect to results from sec 2 (now we add ndcg considerations)
% - interpolate between full overlap to low overlap (random; p(j and j' in list i) same for all j,j' and all i)
% - [explain sampling process: num swaps $N$; converges/mixes at $N \approx 1500$]
%   - [consider labeling x-axis as `\% mixed'
% - usere stdev set to low 0.1; does not encourage div (w/o regularization)
% - in line with prop 1, for $N=0$, get div=0 for all lambda
% - increasing N helps, but more so for larger lambda
% - very sharp div increase/ndcg drop, for relatively small N (=very far from mixed); aligns with prop 2 - need minimal non-overlap to enable high div
% - here we see how ndcg constrains max attainable div (by constraining flex in setting u)
% - [maybe] for higher lambda>0.25, sufficient mixing allows apx max div, but imroved ndcg





%------------------------
\subsection{The role of variation in true user preferences}
\label{variation_u*}
Low user overlap is important, but may not be sufficient 
for promoting diversity when accuracy considerations restrict 
the flexibility in choosing the $u_i$.
When this is the case, we conjecture that the capacity to generate diversity is mediated by the variation in true user preferences $u^*_i$,
since these determine the `directions' in which
accuracy constraints orient embeddings.
To place emphasis primarily on user preferences,
here we consider low-overlap graphs by sampling edges uniformly, using a single time step and setting $\alpha=0$.

Figure \ref{fig:synth} (center) shows NDCG (before strategic updates; bottom) and diversity
(after strategic updates; top), both in absolute values and relative to pre-update diversity,
for varying $\sigma_{u^*}$ and for a range of $\lambda$.
Without regularization ($\lambda=0$),
strategic updates cause diversity to drop to zero,
even when user preferences are reasonably dispersed ($\sigma_{u^*}=1$).
However, even mild regularization ($\lambda=0.05$) suffices obtaining significant diversity through incentivization,
with the effect becoming more pronounced as $\lambda$ grows;
for all $\lambda>0.1$, diversity is high, and in effect remains fixed.
This suggests our model can effectively utilize natural variation in user preferences.
Increased diversity comes at the cost of NDCG, 
but this diminishes quickly for larger dispersion.

\extended{Note that increased preference diversity also naturally promotes NDCG,
as long as some weight is given to accuracy in the objective ($\lambda<1000$).
}

% When user preferences are highly diverse ($\sigma_{u^*}=10$), ...
% 
% \green{
% - w/o reg, div is horrible (=0) until midpoint stdev=1 (=items stdev), then increases (but only slightly above baseline*) \\
% - [div: absolute or relative? relative goes down, so good for us] \\
% - adding regularization gradually helps \\
% - always possible to get div, but at price of ndcg reduction \\
% - price (in ndcg) becomes much smaller for larger dispersion (=higher stdev) \\
% - larger dispersion is better for both ndcg and diversity \\
% - from relatively small $\lambda>0.1$, div stays high and almost fixed, and ndcg increases with dispersion
% }

% \todo{details to appendix: stdev values}




% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.4\textwidth]{synthetic_exp_plots/varying_cost_lam1000.pdf} \qquad
% \includegraphics[width=0.4\textwidth]{angle dispersion.pdf}
% \caption{diversity \textbf{(Left)} and ndcg \textbf{(Right)} over the time.}
% \label{fig:synth cost}
% \end{figure*}


%================================================================
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{real_data_plots/real_data_result_compact_all.pdf}% \qquad
    \caption{
    \textbf{Experiments on Yelp data.}
    \textbf{(Left+center)} Diversity and NDCG over rounds for different methods and target NDCG values,
    for loose ($\alpha=0.1$; left)
    vs. restricted ($\alpha=2.0$; center) strategic updates.
    Our \method{strategic} approach consistently achieves significant and sustained improvement in diversity, with minimal loss in accuracy.
    \textbf{Right} Diversity after $T=10$ rounds
    for increasing costs scales $\alpha$.
    }
    \label{fig:experiements_real}
\end{figure*}
%================================================================

%------------------------
\subsection{The role of time vs. modification costs} \label{sec:synth_vary_costs}
We now turn to examining the temporal formation of diversity
through retraining dynamics, as mediated by modification costs $\alpha$.
When $\alpha$ is large, content creators can only apply small changes to $x$ at each round (and vice versa for small $\alpha$).
On the one hand, small steps suggest that diversity may require time to form; but on the other, note that small steps also allow the system to intervene with high fidelity and direct incentives throughout, which can allow the system to gradually `steer' behavior towards diversification.

% Recall that Prop. \ref{prop:Full_users_overlap}
% showed that full overlap leads strategic updates to decrease diversity to zero, irrespective of system efforts.
% This result, however, is limited to the case $\alpha=0$ in which strategic behavior is unrestricted.
% Here we examine how results can be different under non-zero modification costs.
% When $\alpha>0$, content creators can be thought of 
% as taking small steps over rounds (rather than one big step)
% towards improving their utility.
% In this case, retraining gives the system the power to intervene
% with high fidelity and change incentives throughout.
% In principle, this can allow the system to gradually `steer' behavior towards diversification.
% %  (otherwise unattainable)

Figure \ref{fig:synth} (right) shows post-retraining diversity (top) and NDCG (bottom) 
for increasing $\alpha$ and over multiple retraining rounds.
We set $\lambda$ to be large,
so that the the learning objective is primarily geared towards diversity.
When $\alpha$ is small (here, $<1$), diversity quickly drops to zero---as in Prop. \ref{prop:Full_users_overlap}.
In contrast, $\alpha=1$ exhibits a sharp transition,
in which diversity quickly increases to a large value;
\extended{Fig. \ref{fig:angles} visualizes for a set of items in $\R^2$ how they quickly become dispersed.}
For larger $\alpha$,
diversity reaches similarly high levels;
here the process is slower---since update steps are smaller,
but also more stable---since the system has finer control over each step.
Thus is especially apparent for NDCG, where $\alpha=1$ exhibits large fluctuations
as the system works to preserve diversity by `stepping in place'.


% - (high level: like exp1, want to start from prop1 and extend - but in a different direction)
% - in exp1, $N=0$ is graph of fully-connected components.
% - recall that for $N=0$, div was 0 since we used $\alpha=0$, which means that we cannot generate diversity (since items `jump' to zero); this corresponds prop1 \\
% - when $\alpha>0$, system can incentivize small steps, ie has high-precision control, so can steer trajectory effectively \\
% - study how retraining utilizes this to promote diversity \\
% - set very big $\lambda$ to emphasize div

% results:
% - graph plots ndcg and div after retraining ("consistent")
% - see sharp transition at alpha=1, from div=0 to div reaching 1 (at some point); likely a result of setting $\lambda=1000$
% - alpha=1 reaches high div fast, but is unstable
% - (conversely, larger $\alpha$ takes more time to get high div, but is stable when it does)
% - in ndcg, conjecture fluctuations are means for system to enforce high div by "stepping in place";  
% for alpha=1, which is smallest that still allows high div, steps are large, whereas larger alpha give smaller steps and so smaller fluctuations.



%=================================================================
% \green{\rule{\columnwidth}{3pt}}


% There are several factors that can have an impact on diversity, as we discussed in previous sections. We conducted a series of experiments to examine how diversity is affected by each factor. In this section, all experiments were conducted using synthetic data. Each experiment consists of a recommendation list of 10 items, a system of 50 items, and 200 users. By choosing these options, we could do a realistic experiment in which there are more users than items, and yet the experiment is not too large and can be run quickly. For each user and item, we sample a 2D vector. A sample was taken from two 2D Gaussian distributions in means $\frac{1}{\sqrt{2}}$. Those vectors correspond to the hidden true preferences of each user and the original features of each item. The vectors were normalized to their unit vectors after sampling. To create enough influence on the ndcg (i.e  items should be different from each other before the strategic response), the standard of the items has been set to 1 for the experiments. Using the following score function, we determine the relevance of each item to each user $i$ with hidden true vector preference $u_i$: $rel(x, u_i) = 2^{u^\top x}$.
% \nir{$u$ is the learned embedding - are you using some `ground truth' $u^*$ here? is this what you mean when you say above that you sample 2D vectors for item and *users*?} \itay{Yes}


% \red{state goal - precisely and concisely
% (for example: goal is to understand how and to what degree the natural variation in user preferences affects the system's ability to incentivize/indirectly generate diversity)}



% \subsection{Budget limitation $\alpha$ affects on diversity}
% As we saw in \red{second} experiments, When all items in the recommendation list are belonged to the exactly the same user group (i.e if two items are in the same recommendation list, there is no user that his recommendation list contains only one of those items) and there is no limitation on the cost content creator are willing to pay, the diversity decrease to zero. In addition we saw in the first experiment that it is harder for the model to create diversity when the variance of user hidden true preference is low. In this experiment we show that the price items producer are willing to pay for feature modification might help the model create diversity. Intuitively when the $\alpha$ is 0 the model has fully control about items movement. However in this experiment we empirically show that the model can use the budget limitation to create diversity even in those extremes condition. Thus, we set user true preference std to $0.1$ and the items user graph to be as same as the second experiment (without any replacement between items groups). In order to see how item change over times, in this experiment we sample items from two 2D Gaussian distributions in means $\frac{-1}{\sqrt{2}}$ which is the farthest from the user preference means. In addition we used for sampling smaller std than used in previous experiments ($0.25$ instead of $1$ ) we used smaller std since we wanted to emphasize how the model create diversity over the time (due to small std the initial diversity is low). In order to show how the how diversity is created over the time from different values of $\alpha$ we repeated this experiment 150 times. The result of $\lambda=1000$ are presented in Fig. \ref{fig:synth cost}. We chose this value since it very high and tries to increase diversity with tinny care about ndcg. As we can see, for small value of $\alpha$ (includes 0) the model doesn't succeed create diversity. When $\alpha$ gets higher the model can break the items movement and in each change increase the diversity until it gets to high point. When high diversity is achieved model should change user embedding in order to maintain the diversity. Such a change probably cause decrease in NDCG. In figure \ref{distribution over time 1 rec list} we observe how the RS maintains the diversity over the time. The dots in the plot represents item fro m the same recommendation list. Colors are assigned to each item. We can observe the periodic structure that used by the RS to maintain the diversity.   \red{should I switch the scatter time dots plots with another plot that all dots there are in same recommendation list and each dot has a unique color? that might be}

% \begin{figure*}[t]
%   \includegraphics[width=\linewidth]{synthetic_exp_plots/distribution_time_c1.pdf}
%   \caption{$\lambda=1000$, $ \alpha=1$}
%   \label{distribution over time all data}
% \end{figure*}
% \begin{figure*}[t]
%   \includegraphics[width=\linewidth]{synthetic_exp_plots/distribution_time_c1_one_rec_list.pdf}
%   \caption{$\lambda=1000$, $ \alpha=1$}
%   \label{distribution over time 1 rec list}
% \end{figure*}

% \begin{figure*}[t!]
% \centering
%     \begin{subfigure}[b]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{synthetic_exp_plots/div_cost_lam1000.pdf}
%     \caption{\red{todo}}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{synthetic_exp_plots/ndcg_cost_lam1000.pdf}
%     \caption{\red{todo}}
%   \end{subfigure}
%   \label{synth cost}
% \end{figure*}
% \todo{state conclusions - what is the main statement?}
